The Early Bird Catches the Leak: Unveiling Timing Side Channels in LLM Serving Systems

The wide deployment of Large Language Models (LLMs) has given rise to strong demands for optimizing their inference performance. Today's techniques serving this purpose primarily focus on reducing latency and improving throughput through algorithmic and hardware enhancements, while largely overlooking their privacy side effects, particularly in a multi-user environment. In our research, for the first time, we discovered a set of new timing side channels in LLM systems, arising from shared caches and GPU memory allocations, which can be exploited to infer both confidential system prompts and those issued by other users. These vulnerabilities echo security challenges observed in traditional computing systems, highlighting an urgent need to address potential information leakage in LLM serving infrastructures. In this paper, we report novel attack strategies designed to exploit such timing side channels inherent in LLM deployments, specifically targeting the Key-Value (KV) cache and semantic cache widely used to enhance LLM inference performance. Our approach leverages timing measurements and classification models to detect cache hits, allowing an adversary to infer private prompts with high accuracy. We also propose a token-by-token search algorithm to efficiently recover shared prompt prefixes in the caches, showing the feasibility of stealing system prompts and those produced by peer users. Our experimental studies on black-box testing of popular online LLM services demonstrate that such privacy risks are completely realistic, with significant consequences. Our findings underscore the need for robust mitigation to protect LLM systems against such emerging threats.

==> tex/discussion.tex <==
\section{Discussions}

%\para{Bridging the gap to real world}

%\link{Review D: While the authors could have chosen a local setup due to ethical considerations, they still need to provide a stronger argument for how and why these local setups and configurations are representative of real, remote LLM services, and how the results obtained from local setups could translate to real-world attacks against production systems.}
% Choice of Open-Source Framework: We used one of the most well-known open-source LLM serving frameworks, which is widely adopted in production environments. This choice ensures that our setup reflects the core mechanisms and security measures of real-world systems.

%Similarities and Differences: We conducted a thorough analysis of the similarities and differences between our local setup and real-world LLM services. Our setup captures essential behaviors and vulnerabilities relevant to our study, while acknowledging that production environments may have additional security layers and scalability features.

%Generalizability of Findings: We provided evidence and reasoning to support the generalizability of our findings. This includes discussing how the attacks studied exploit fundamental design flaws likely present across different implementations.

%Ethical Considerations: We emphasized the ethical considerations of using a local setup, highlighting its role in responsible research practices aimed at improving security without enabling misuse.

%Threat Model and Counterarguments: We included a threat model to specify the assumptions and scope of our study, and addressed potential counterarguments regarding optimizations or security patches in production systems.

%Additional Experiments and Industry Insights: We considered running additional experiments and sought insights from industry experts to further validate our findings in controlled production environments.


%\link{Some differences and obstacles: not stable network latency, etc..}


\para{Co-locations}
Co-location is a prerequisite for timing side-channel attacks. There has been significant research on how to achieve co-location in the cloud for micro-architectural side channels~\cite{ristenpart2009hey,zhenyu2012whispers,zhang2014cross,varadarajan2015placement}. Co-location can be more efficient in LLM systems because these systems often focus on optimizing cache reuse through improved scheduling policies. 
For example, baseline scheduling policies, such as first-come-first-serve, typically do not consider the shared prompts within an LLM system. As a result, requests may be mixed across different LLM engines, preventing the reuse of common prompt prefixes and potentially leading to suboptimal cache efficiency. To address this, LLM serving systems like SGLang~\cite{sglang-github}, Parrot~\cite{lin2024parrot}, Mooncake~\cite{qin2024mooncake} and BatchLLM~\cite{zheng2024batchllm} have introduced modified schedulers that prioritize requests that align with cached prefixes, a strategy known as cache-aware scheduling.

\noindent\textbf{Unexplored timing leakages.}
This paper utilizes SGLang~\cite{sglang-github} and GPTCache~\cite{gptcache-github} as the most representative KV cache and semantic cache sharing mechanisms. However, it is important to note that more sophisticated optimization techniques may enhance performance, but they could also amplify the significance of timing leakage.
For example, modular prefix caching~\cite{gim2024prompt} and CacheBlend~\cite{yao2024cacheblend} facilitate KV caching for not only prefix tokens but also intermediate ones. Cascade inference~\cite{cascade-inference} stores the shared KV cache in GPU shared memory (SMEM for short), for fast access in multiple requests. The sharing of KV cache in speculative decoding~\cite{leviathan2023fast} may also introduce speculative side channels, akin to Spectre~\cite{kocher2020spectre}.
%Besides, this paper only considers shared public LLM services. Sharing KV caches may also occur on local deployed LLMs with the trend of LLM as an OS~\cite{mei2024aios}. 
We leave the further exploration of the impact of the discovered side channels to future work.

\para{Real-world attacks}
In real world attacks, especially targeting online LLM services, the network latency will bring additional noises to the timing. The noise effect could be reduced with more attack trials. Besides, it has been shown possible to mount cache attacks from the remote network~\cite{kurth2020netcat,schwarz2019netspectre}.

\ignore{
\subsubsection{Sharing non-prefix KV cache}
CacheBlend source code: \url{https://github.com/YaoJiayi/CacheBlend}

when an LLM input includes multiple text chunks, how to quickly combine their
precomputed KV caches in order to achieve the same generation quality as the expensive full prefill?

We present CacheBlend, a system that fuses multiple
pre-computed KV caches, regardless of prefix or not, by
selectively recomputing the KV cache of a small fraction of
tokens, based on the preceding texts in the specific LLM
input.

To put CacheBlend in context, our contribution lies in
enabling the reusing of KV caches of multiple text chunks in
one LLM input, without compromising generation quality

\textcolor{red}{@Zixuan}

\wenhao{try to recover the prompt template; it may not be possible but we can have a try}




%\subsection{Others}
%performance downgrade attacks by abusing the speculative decoding

%Abusing other vLLM strategies?
%The blocks whose ref counts reach zero are freed
%Eviction policy (e.g., grouping eviction)
%Scheduling policy

%\para{Evaluations}


\subsubsection{Sharing KV cache in backbone model of LoRA}
LowRank Adaptation (LoRA)
\wenhao{the attacker and victim may query different models, but as long as the backbone model is the same, there should exist observable timing difference}\textcolor{red}{@Linke}

\textcolor{red}{it may not be possible but we can have a try}

S-LoRA: Serving thousands of concurrent LoRA adapters~\cite{sheng2023s}
}

%\subsubsection{Co-locations}

%Achieving co-location is crucial for timing side-channel attacks. Extensive work has been undertaken to comprehend how to achieve co-location in the cloud for micro-architectural side channels, such as cache side-channel attacks~\cite{}.
%We have discovered that achieving co-location more efficiently is possible, as existing LLM systems strive to enhance cache reuse through optimized scheduling policies.

%The baseline scheduling policy, such as first-come-first-serve, is not aware of the shared prompt within each LLM platform, the requests are mixed in all LLM engines making it impossible to reuse the common prompt prefix, and may lead to sub-optimal cache reuse. Therefore, LLM serving systems such as RadixAttention~\cite{}, Parrot~\cite{lin2024parrot} and Mooncake~\cite{} provides the modified scheduler which prioritizes requests that match cached prefixes, known as cache-aware scheduling.

%\para{Experiment validations}

%Our testbed is equipped with 4 Nvidia A100 cards. 

%\textcolor{red}{@linke}
%\para{RadixAttention}
%Optimal cache reuse may not be compatible with schedules such as first-come-first-serve. 
%RadixAttention therefore comes with a modified scheduler which prioritizes requests that match cached prefixes (cache-aware scheduling).

%The scheduling policy could be used to create timing difference, which leaks the prompt information.
%\wenhao{Assuming the system load is almost full, we send a chunk of different prompts, if any prompt responses sooner than the others, it is more likely that it hits the cache (caused by scheduling)}\wenhao{we need to benchmark GPTCache}
%\wenhao{Parrot may be more suitable for the case of prefix sharing}
%Llumnix: Dynamic Scheduling for Large Language Model Serving

%Fairness in Serving Large Language Models

\ignore{
\para{Parrot: Efficient Serving of LLM-based Applications with Semantic Variable~\cite{parrot}}
Currently, most LLM-based
applications exhibit a high degree of redundancy in the
prompts of their requests. For instance, Bing Chat~\cite{} has
handled more than 1 billion chat prompts. These prompts
share the same system prompts that defines the functionality
of Bing Chat. OpenAI introduces GPTs~\cite{} to let users customize a ChatGPT for a specific purpose whose prompt template is the same across users.
\wenhao{Parrot supports placeholders in a prompt}

Parrot maintains a key-value store,
where each entry maps a (hashed) prefix of tokens to a list of
requests, thus the scheduler can quickly check the opportunity
in an online manner, supporting both static and dynamically generated prompt within one application or even across different applications. Furthermore, we propose better GPU kernel for the attention computation of the requests with a common prefix. We
first leverage vLLM's paged memory management to
save the redundent GPU memory. But vLLM's kernel still
suffers from redundant computation and memory loading
of the shared tokens. Therefore, we design a new Attention
decoding algorithm by combining FlashAttenation and
PagedAttention that treat the shared and non-shared token separately. This significantly accelerates the attention of
shared contexts.

OpenAI ChatML~\cite{}

\url{https://github.com/openai/openai-python/blob/e389823ba013a24b4c32ce38fa0bd87e6bccae94/chatml.md}

Because the
baseline's scheduling policy is not aware of the shared prompt
within each LLM application, the requests are mixed in all
LLM engines making it impossible to reuse the common
prompt prefix. Parrot's scheduling policy co-locates LLM
requests of the same applications to maximize the sharing opportunity, achieving both lower inference latency and higher
cluster throughput.
}
%\wenhao{no leakage, but it shows requests with common prefix may be scheduled to the same LLM engine}
%\wenhao{we'd better benchmark this claim too}

%\subsection{Routing policy in MoE}

%\wenhao{routing to different expert etc., based on the input characteristics} However, it's usually not clear how it is routed, even for open-sourced MoE

%\subsection{Model Compression}


%\subsection{Speculative decoding}
%\wenhao{see comments}
% 有可能会出现类似Spectre的timing side channel，但是条件要求比较高，原因为：draft model接受多个用户的输入，每个draft model产生的draft token会送到verification model，在verification model进行类似于prefill阶段的验证。

% 若verification的prefill阶段可以复用kv cache，则可以通过构造输入mis-direct the draft token产生特定的draft token，再根据draft token返回的timing difference，推测其它用户是否有类似的draft token，进而推测其它用户的输入

%\subsection{LLM-based applications}
%To accomplish a task, LLM-based applications typically
%require multiple rounds of conversation. The conversation, implemented through multiple API calls to LLM, demonstrates complex workflow patterns.

%For example, a meeting summary application often divides a lengthy document into multiple shorter sections, each satisfying the length constraint of the LLM conversation and thus can be summarized and combined into the final summary through the Map-Reduce or chaining summary patterns. Chat-based applications, e.g., Bing Copilot, call LLM APIs multiple times to generate answers based on user queries. Multiple agents, each representing a different role played by different LLM calls, can collaborate to achieve a task.

%There exist significant opportunities to improve the end-to-end experience of LLM applications by exploiting the application-level information, especially the correlation of multiple LLM requests~\cite{lin2024parrot}. First, multiple consecutive LLM requests may be dependent: the result of one request could be the direct input of the next request. Therefore, it is desirable to colocate those requests together and execute them consecutively on the LLM service side. Second, there exists a high degree of commonality across LLM requests. Popular LLM applications use a long system prompt, including task definitions, examples, and safety rules, to guide the behavior of LLM applications. The long system prompt is usually static and common for all users. As existing public LLM services treat each request individually, these common prefix prompts are provided repeatedly in each request, leading to a great waste of storage, computation, and memory bandwidth. Our
%analysis of a production LLM-based search engine shows that over 94\% of tokens in the requests are repeated across different users.

%There have been several frameworks for developers to build LLM-based applications, e.g., LangChain, SemanticKernel,
%and PromptFlow. The key function of these frameworks
%is to “glue” different LLM calls to accomplish a complex
%task (aka. LLM orchestration). Most of these frameworks
%have already used a template-based approach in which developers can design a template with placeholders, and render the placeholders at runtime. These placeholders naturally have the same concept as Parrot's Semantic Variable. 

==> tex/ethics_and_open_science.tex <==
%\newpage
\section*{Ethical Considerations \& Disclosure}
We follow standard best practices to ensure that our study follows ethical principles~\cite{kohno2023ethical}. The evaluations were performed in a controlled local environment. All targeted system prompts or user prompts are collected from public data without any personal information.
In the black-box measurement of online LLM services, we only send prompts and receive responses. In this process, we only infer whether our own requests are cached by observing the response latency. We do not intend to recover the system prompt or private prompt with the discovered side channel for these online services.
As this study is based on publicly available data and does not involve any human participants, it is not considered as human subjects research by our Institutional Review Boards (IRB).

While publishing our results can raise concerns about misuse, we believe that raising awareness of the problem is even more important, as it can inform LLM vendors and the research community to build more robust systems.
We have reported our findings to all the developers (SGLang, GPTCache etc.), and LLM service providers (OpenAI, Claude and Google Gemini etc.) as soon as we identified the side channels.
Our reports were delivered via the official security report portal or by separate e-mails.
As of the preparation of this manuscript, they were still investigating this issue, and we remain in communication with them.



%report to OpenAI/Claude etc.

%website


\section*{Open Science}
%All the code and dataset to reproduce our experiments are available at \url{https://anonymous.4open.science/r/llm-sidechannel-AE16}. 
%We release the code for review purposes. If it raise concerns about misuse, we will remove it from public access.
We will make all the code and datasets required to reproduce our experiments publicly available after the paper is published.

% https://bughunters.google.com/

% https://bugcrowd.com/openai

%  disclosure@anthropic.com for Claude

==> tex/eval_backup.tex <==
%\section{Leakages Exploration in Local Environment}
\section{Evaluation}
\label{sec:eval}

%\wenhao{we need to provide as many case studies as possible}

%In this section, we present an empirical evaluation of the characteristics of the discovered side channels, and elaborate on how to exploit them efficiently. To reduce the impact on innocent users of public LLM services, we built the system in the local environment using open-sourced projects, trying to replicate real-world deployment of LLM serving systems.

In this section, we provide an empirical analysis of the identified side channels and outline strategies for their efficient exploitation. To prevent disruptions to public LLM services,
we built the system in the local environment using open-sourced projects, trying to replicate real-world deployment of LLM serving systems. 
%\subsection{Experiment Setup}

% Intel(R) Xeon(R) Silver 4310 CPU @ 2.10GHz
%we replicated real-world deployment scenarios by conducting experiments locally using open-source projects.} %To reduce the impact on innocent users of public LLM services,} 

%All our local experiments were conducted on a Lenovo server equipped with an Intel(R) Xeon(R) Silver 4310 CPU (running at 2.10 GHz with 12 cores) and 500 GB of DDR4 memory. The system is equipped with 4 NVIDIA A100 GPUs (each with 40 GB of GPU memory).  
All the experiments were conducted on a Lenovo server with two Intel Xeon E5-2678 v3 CPU (12 cores, 2.50 GHz), 100 GB DDR4 memory, and 2 NVIDIA A100-PCIE GPUs (40 GB memory each). The system ran the Ubuntu 22.04 (kernel 5.15.0-125-generic) OS with GPU driver 550.127.05, CUDA 12.4, and PyTorch 2.4.0. Open-source models, particularly from the Llama family, were used as the underlying LLM. All evaluations were performed using the default configurations for both hardware and software settings.
%\wenhao{@link: update the configuration}

%All our local experiments were conducted on a Lenovo server equipped with an Intel(R) Xeon(R) CPU E5-2678 v3 CPU (runing at 2.50GHz with 48 cores) and 500 GB of DDR4 memory. The system is equipped with 4 NVIDIA A100 GPUs (each with 40 GB of GPU memory).
%The system runs on Ubuntu 18.04 OS (kernel version: 5.4.0-150-generic), with GPU driver version 525.125.06, CUDA 11.8, and PyTorch 2.3.1.  

%We used open-source models, including LLM family like Llama, Qwen, etc. \link{May need to update.} Both the server and client were deployed on the same server, communicating through the local loopback network interface.

%We performed local experiments under two configurations: (1) assuming no network latency, with both the server and user running on the same machine and communicating via the local loopback interface; and (2) simulating communication between the server and user located on separate nodes within the same local area network (LAN).
%\hl{We tested two configurations: (1) a no-latency setup, with the server and user running on the same machine and communicating via the local loopback interface, and (2) a simulation of communication between the server and user on separate nodes within the same local area network (LAN).}

%\link{We've changed the setting according to Reviewer C, but we need to emphasis why using 2 is still easy and handy.}
%Both the server and client are deployed on the same machine, communicating over the local loopback network interface.
%Hardware: CPU/GPU/Memory



%Datasets: what datasets are used for the experiment validations
%\wenhao{chatbot dataset: ShareGPT}

% yet for the web mode, we still don't have lanuch related labs.
%In the API mode, we get the latency through timer function of python (), while in the web mode, we get the latency through xx.

%Software: OS/GPU driver/CUDA/Pytorch

%In our evaluation, we used two publicly available datasets: ShareGPT~\cite{sharegpt-website} as the chatbot dataset, and xx~\cite{} as the xx dataset.

%Some medical question-answering benchmarks are derived from medical entrance and licensing exams, such as
%MedMCQA~\cite{pal2022medmcqa} and MedQA~\cite{zhang2018medical}. MedQA, for example, is based the US Medical Licensing Exam (USMLE)~\cite{usmle-website}.


\subsection{Prompt Stealing Attacks (PSA) on System Prompt}
\label{subsec:evalpsa}


\subsubsection{Attack overview}

%\hfill\\

As outlined in \autoref{subsec:threat_model}, we consider a scenario where a victim user creates a popular LLM application (e.g., a chatbot) using a proprietary system prompt via a public API service (e.g., the OpenAI API). The attacker aims to steal this system prompt by querying the LLM APIs.
For this evaluation, we focus on a specific use case built with open-source projects. Specifically, the public API service is implemented using the backend API server of SGLang~\cite{sglang-github}, which supports KV cache sharing for common prefixes, while the victim's LLM application is built with the FastChat~\cite{zheng2023judging} framework.

LLM APIs typically allow users to define different roles, such as ``system'' and ``user'' in their input. The complete prompt sent to the LLM is formed by concatenating the messages associated with each role, following predefined templates (\autoref{fig:system_prompts}). In this case, we assume the victim's chatbot uses a proprietary system prompt as the message for the ``system'' role, while user inputs are associated with the ``user'' role. Following the prompt template, the system prompt is repeatedly prepended at each conversational turn to form the complete prompt sent to the SGLang backend API server.

As shown in \autoref{fig:model_PSA}, an attacker acting as a user of the chatbot can send either a direct query or a synthesized request that includes the fixed system prompt. When the LLM processes these synthesized prompts, it stores the separator and system prompt in the KV cache managed by the SGLang backend. This enables subsequent direct queries, which use partial prefixes of the separator and system prompt, to benefit from faster responses.
Thus, the attacker first uses the synthesized request to keep the targeted system prompt in the KV cache, then crafts specific direct queries to leak the system prompt by observing timing differences.

%By using synthesized requests, the attacker can keep the system prompt in the KV cache and infer it through direct queries.


%Taking FastChat as an example, the fixed system prompt is repeatedly prepended at each conversational turn. Notably, these chatbots allow users to either send prompts directly to the LLM or construct complete requests using the \textbf{LEGO} shown in \autoref{fig:system_prompts}, in an OpenAI-compatible API manner~\cite{Send_request}.

%While the detailed use of system prompts in proprietary software is unclear, we reviewed the code of widely adopted open-source chatbot frameworks including FastChat~\cite{zheng2023judging} and SGLang~\cite{sglang-github}. 

%As illustrated in \autoref{fig:system_prompts}, these systems typically integrate the system prompt with the user prompt either as a prefix or via a model template, forming the complete prompt sent to the LLM. Additionally, the content of the system prompt can be fixed or customized.

%\link{The persistence of the System Prompt within the conversation context needs to be further discussed.}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/system_prompts.pdf}
    \caption{Synthesis of complete prompts.}
    \Description{}
    \label{fig:system_prompts}
\end{figure}

\ignore{
Open-sourced chatbots typically input the system prompt once at the start or repeatedly throughout each conversation. While inputting it once at the begining may be efficient, when token count increases or malicious input occurs, system prompt data may be evicted, leading to disruptions or security risks like jailbreaking~\cite{liu2023jailbreaking}. To mitigate this, services like FastChat rely on a fixed system prompt for gpt-4-turbo or claude-3-sonnet~\cite{fastchatsrc}, which is repeatedly prepended at each conversational turn to maintain stability. Notably, these chatbots allow users to either send prompts directly to the LLM or construct complete requests using the \textbf{LEGO} shown in \autoref{fig:system_prompts}, in an OpenAI-compatible API manner~\cite{Send_request}.


Based on these findings, we devised an end-to-end attack model in \autoref{fig:model_PSA}. We assume the victim deploys a chatbot via SGLang with a fixed prompt and default chat template of selected model. An attacker, acting as a user, can either send a direct query or a synthesized request containing the fixed system prompt. Upon processing the synthesis prompts, the LLM will store the KV cache of seperator and system prompt in the backend, enabling subsequent direct queries with partial prefixes of the separator and system prompt to benefit from accelerated responses, as reflected in TTFT. Thus, attackers may use synthesized requests to keep the system prompt in the KV cache and infer it through direct queries.

While the separator under a default chat template of the selected model is finite and can be revealed, reconstructing the victim’s secret system prompt remains challenging due to its infinite possible variations. We assume the initial tokens can often be statistically guessed, such as starting with "You are...". Attackers focus on system prompts closely aligned with their interests, testing their relevance to their objectives before proceeding further, while disregarding prompts with minimal semantic similarity to their goals.
}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/PSA.pdf}
    \caption{End-to-end model of prompt stealing attacks.%\wenhao{the arrows are confusing: it's hard to understand where to start and where to end}\link{I will fix it.}
    }
    \Description{}
    \label{fig:model_PSA}
\end{figure*}

\subsubsection{Characterizing the leakage}
\label{subsubsec:chrctpsa}

%\hfill\\


%Hydragen: High-Throughput LLM Inference with Shared Prefixes
%Relayattention

%https://github.com/rayleizhu/vllm-ra

%All-or-nothing eviction policy: either evict all or none of the blocks of a prompt sequence

% 我们采用了基于SGLang推理框架的后端系统，对不同权重的llama2模型进行实验。本实验的目标是评估在单卡环境下，前缀匹配长度对模型处理速度，如first token time（FTT）的影响。为此，我们设计了一系列实验，验证不同长度前缀在部分命中与完全未命中情况下对FTT的影响，并分别选取了9000条长度一致的prompt样本计算LLM响应时间。

% 根据图中的实验结果所示：随着前缀命中长度的增加，模型在FTT上表现出显著的时间缓存效果，在权重较大的模型中，这种效果更为明显和稳定。由于70B模型上处理单个 token 所需的时间更长，GPU显存占比也更大，所以前缀缓存带来的时间减少效果也会更加显著，可以在token级别观察到。

% 在此基础上，我们的实验进一步证明了存在时序侧信道泄露。 利用不同前缀长度条件下，前缀hit与miss情况下收集的FTT数据，我们设计并训练了一个高效的分类器。该分类器能够判断输入的时间数据是否属于前缀命中的FTT类别。根据验证集测试，分类器可以达到70%的准确度，这表明了攻击者可以利用这一泄露来推断prompt的前缀匹配情况。

% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/13b.pdf}
%         \caption{llama2-13B}
%         \label{fig:llama13b}
%     \end{subfigure}
%     %\hspace{5pt}
%     \hfill
%     \begin{subfigure}{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/70b-gptq.pdf}
%         \caption{llama2-70B-GPTQ}
%         \label{fig:llama70b}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/70b-gptq.pdf}
%         \caption{llama2-70B-GPTQ}
%         \label{fig:llama70b}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/70b-gptq.pdf}
%         \caption{llama2-70B-GPTQ}
%         \label{fig:llama70b}
%     \end{subfigure}
%     \caption{Leakage profile of sharing the KV cache. We used two models with different sizes: \texttt{llama2-13B} and \texttt{llama2-70B-GPTQ}, and plotted the ROC curve to fingerprint the timing difference when the prompts share the prefix of 1, 2, 4 and 8 tokens respectively.}
%     \label{fig:leakage_kv}
% \end{figure*}

\ignore{
\textcolor{red}{However, latency distributions for hit and miss cases might still overlap, making classifier of simple thresholds ineffective. Based on the experimental conditions outlined in \autoref{sec:eval}, we present latency distributions for cases where the shared-prefix token count differs by one or two, corresponding to cache hits and misses, with 1,000 tests per sample. The \autoref{fig:distribution} shows that single-token hits and misses are indistinguishable without special handling, while two-tokens differences, though overlapping, can be distinguished.}
}


\begin{figure}[!ht]
    \centering
    % \begin{subfigure}{0.24\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/llama-2-13b-hf.pdf}
    %     \caption{LLaMA-2-13B-hf}
    %     \label{fig:llama-2-13B-distribution}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/8B-instruct-onetoken.pdf}
        \caption{LLaMA-3.1-8B-Instruct}
        \label{fig:llama-3.1-8B-distribution}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/70B-onetoken.pdf}
        \caption{LLaMA-2-70B-GPTQ}
        \label{fig:llama-2-GPTQ-70B-distribution}
    \end{subfigure}
    \caption{Latency distribution of one token hit and miss. We used 2 representative models of different sizes: \texttt{llama3.1-8B-Instruct} and \texttt{llama2-70B-GPTQ}. We will use the \texttt{llama2-70B-GPTQ} model for subsequent evaluations. %\wenhao{we should remove the first figure, which shows no timing difference, or replace it with another one; besides, we should state which model is used for subsequent evaluations}
    }
    \Description{}
    \label{fig:distribution}
\end{figure}

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=.95\linewidth]{figures/leakage_kv.png}
% \caption{Leakage profile of sharing the KV cache. We used two models with different sizes: \texttt{llama2-13B} and \texttt{llama2-70B-GPTQ}, and plotted the ROC curve to fingerprint the timing difference when the prompts share the prefix of 1, 2, 4 and 8 tokens respectively.}
% \label{fig:leakage_kv}
% \end{figure*}

\para{Timing distributions}
First, we investigate the impact of different token sharing lengths on the model's timing characteristics. We evaluated SGLang v0.3.0~\cite{sglang-github}, which organizes KV cache blocks into a radix tree for efficient prefix matching and KV cache reuse. Our experiments focused on how matched prefix token lengths affect response latency (i.e., TTFT) in a single-GPU environment, using the llama3.1-8B-Instruct, and llama2-70B-GPTQ models.
Prompts of varying prefix lengths were generated from the \path{gabrielchua/system-prompt-leakage}~\cite{systemprompt-huggingface} system prompt dataset from Hugging Face~\cite{systemprompt-huggingface}. %which contains over 350,000 synthetic system prompts of different lengths.
{We present latency distributions for cases where the shared-prefix token count differs by one, corresponding to cache hits and misses, averaged over 4,000 runs for every test case. As shown in \autoref{fig:distribution}, for LLaMA-2-70B-GPTQ, the difference between hit and miss is notably distinct, with negligible overlap, enabling their separation via a simple threshold.}%single-token hits and misses are indistinguishable without special handling, while two-token differences, although overlapping, can be distinguished.}

%\link{Maybe we can use even more LLM here.}
%For this evaluation, we used SGLang v3.0.0~\cite{sglang-github} as a representative system. SGLang reorganizes the KV cache blocks into a radix tree to support efficient prefix matching and KV cache reuse. We conducted experiments to measure the correlation between the token length of matched prefix and the response latency of the model (i.e. TTFT in the single-GPU environment) on llama2-13B and llama2-70B-GPTQ models. 
%\textcolor{red}{We evaluated SGLang v3.0.0~\cite{sglang-github}, a widely adopted LLM serving framework in the open-source community with significant influence in both industry and academia~\cite{SGLang_AMD, yang2024copsempoweringllmagents, gptqmodel}. SGLang enhances efficiency by reorganizing KV cache blocks into a radix tree, enabling effective prefix matching and KV cache reuse.}


 %\link{Change the Dataset, and Remember to describe the dataset, why we choose to use this one?} 

 
% 下面这个部分需要搬到后面去
%\link{Not Sure about that, or we should conduct an expriment to ensure this argue. The Experiment is doing now. After some experiments, I am sure that the token counts a lot. So it is also a challenge we should mentioned afterwards.} Furthermore, we confirmed that the content of the prompts had no substantial effect on response latency.

% Our experiments were designed to evaluate the relationship between the matched prefix length and the model's response latency (i.e., TTFT in the single-GPU environment. We have conducted the evaluation on two models, namely llama2-13B and llama2-70B-GPTQ, to investigate how the model size influences the timing leakage.
% \link{The aim of the investigation is unclear. Better to have a clear aim, or we should delete}

%We used the public system prompt dataset~\cite{systemprompt-website} to generate prompts with different lengths of matched prefix. Besides, we confirmed that the content of the prompt did not result in noticeable differences in the response latency.

%We randomly choose one target system prompt $T$ from the dataset and truncated its prefix with token lengths of 4, 5, 7, 11 to obtain four different prefixes. We assume %

% remove figure 4 for now
\ignore{
To assess the impact of the shared prefix token length on the response latency, %in the \textit{first} step, 
we generated five groups of prompts of the same length as $T$, and the groups were denoted as $T_0$, $T_1$, $T_2$, $T_4$,and $T_8$, which shared exactly the initial $k$ tokens with $T$ for $k = 0, 1, 2, 4,$ and $8$, by replacing the $(k+1)$-th token with different tokens in each group. \textcolor{red}{Each group consisted of 2000 prompts, and TTFT was measured for each prompt immediately after $T$ was processed and cached by the LLM. Prompts from $T_0$ (no shared prefix with $T$) were labeled as $0$, while those from groups with shared prefixes (lengths $1, 2, 4, 8$) were labeled as $1$. }

\begin{figure*}[!ht]
    \centering
    \begin{subfigure}{0.33\linewidth} % 宽度设置为0.24\linewidth，确保四个图在同一行
        \centering
        \includegraphics[width=\textwidth]{figures/roc_test_LLaMa-3.1-8B.pdf}
        \caption{llama3.1-8B-Instruct}
        \label{fig:llama13b}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/13b.pdf}
        \caption{llama2-13B}
        \label{fig:llama70b}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/70b-gptq.pdf}
        \caption{llama2-70B-GPTQ}
        \label{fig:llama70b_2}
    \end{subfigure}
    %\hfill
    % \begin{subfigure}{0.24\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/70b-gptq.pdf}
    %     \caption{llama2-70B-GPTQ}
    %     \label{fig:llama70b_3}
    % \end{subfigure}

    \caption{Leakage profile of sharing the KV cache. We used three models with different sizes: \texttt{llama3.1-8B-Instruct}, \texttt{llama2-13B} and \texttt{llama2-70B-GPTQ}, and plotted the ROC curves to fingerprint the timing difference when the prompts share the prefix of 1, 2, 4, and 8 tokens respectively.\link{These three graph Maybe all need to be updated. I am afraid we might use other form instead of ROC curves.}}
    \label{fig:leakage_kv}
\end{figure*}

%Next, for each prompt within the group, we measured the TTFT when these prompts were fed into the LLM, right after $T$ was fed into the LLM and was cached. In our evaluation we set the group size to $2000$, and designated the collected samples from group $T_0$ (i.e., no shared prefix with $T$) as $0$, and the collected samples from other groups (i.e., shared prefixes of lengths $1, 2, 4, 8 $ with $T$) as $1$. Finally, 
%we trained a set of classifiers based on the collected samples to determine whether a prompt misses the prefix cache or hits the prefix cache matching the corresponding length. We then 
\textcolor{red}{\autoref{fig:distribution} reveals timing differences from a few tokens are negligible, with overlapping latencies in distribution. To separate $T_0$ from other prompt sets, we used ROC curves, which illustrate the trade-off between false positive rate (FPR) and true positive rate (TPR), to effectively capture timing differences. \autoref{fig:leakage_kv} demonstrates that longer shared prefixes significantly enhance TTFT caching, with larger models showing a stronger and more stable effect.} %We plotted the ROC curves for all datasets to visualize the timing difference in \autoref{fig:leakage_kv}.
%The results clearly demonstrate that as the length of the shared prefix increases, the model exhibits a significant caching effect on TTFT. This effect is more pronounced and stable in larger models.
%Given the extended processing time for a single token on the 70B model and the higher GPU memory usage, the time reduction effect facilitated by the prefix cache becomes more substantial. This effect is observable at the token level.
}


%For demonstration purposes, we used the llama2-70B-GPTQ model for our subsequent evaluation. Our classifier uses an XGBoost model, with Bayesian optimization used to determine the best parameters.
%According to the test on the validation dataset, the classifier can achieve an accuracy of 70\%, which indicates that the attacker can use this leakage to infer whether the prompt matches the target prompt in the KV cache.
%\wenhao{@zixuan, redraw the picture}


%uring the AUC calculation, the response time labels for prefix hit prompts are set to 1, and for prefix miss prompts, they are set to 0. Finally, we plot the ROC curves for both.To quantify the leakage, we report the AUC-ROC curves of 5 random trials.

%Our selection of system prompts from the system_prompt dataset involved replacing a word at a specific position k with 9000 random words. The text preceding this altered word was deemed a k-length prefix match. These generated prompts were categorized as prefix hit data. Conversely, prompts of the same length but with the initial k words differing from the target system prompt were categorized as prefix miss data. Subsequently, we calculated the response times for these two categories when fed into the LLM.



%We designed a series of experiments to verify the impact of prefixes of different lengths on TFTT in the cases of partial hit and complete miss, and selected 9000 prompts of consistent length to calculate the response time of LLM and plot the relationship between false positive and false negative. 
%We selected system prompts from the system\_prompt dataset, replacing a word at a specific position k with random 9000 words. The text preceding this word is considered a k-length prefix match. These generated prompts are classified as prefix hit data, while other prompts of the same length but with the first k words differing from the target system prompt are classified as prefix miss data. We then calculate the response times for these two categories when input into the LLM. During the AUC calculation, the response time labels for prefix hit prompts are set to 1, and for prefix miss prompts, they are set to 0. Finally, we plot the ROC curves for both.To quantify the leakage, we report the AUC-ROC curves of 5 random trials.

%Finally, according to the experimental results shown in the Figure~\ref{fig:leakage_kv}: with the length of the prefix match increases, the model shows a significant time caching effect on TFTT, and this effect is more pronounced and stable in models with larger weights. Due to the longer time required to process a single token on the 70B model and the larger GPU memory occupancy, the time reduction effect brought by the prefix cache will be more significant and can be observed at the token level.

%On this basis, our experiment further proves the existence of a temporal side channel leak. Using the TFTT data collected under different prefix lengths in the hit and miss conditions of the prefix, we designed and trained an efficient classifier. This classifier can determine whether the input time data belongs to the TFTT category of the prefix hit. According to the test on the validation set, the classifier can achieve an accuracy of 70\%, which indicates that attackers can use this leak to infer the prefix matching situation of the prompt.
% use SGLang as a representative system, use llama-13B and llama-70B-4bit for this evaluation. train a model, and 

% Firstly, explain how the evaluation was conducted, then the results

% finally, what we learn from the results

%\link{Express the Basic challenge here.}

% \para{Challenges of Attacks}

% \link{Several Challenges: few tokens, Length, classifier training sentences.}

% Unstable timing: the position and the method to record the latency(Might not enough to put into the paper)

% Length: Not a problem. Same case for eviction and flush.

\para{Building the classifier to recover 1 token}
%While the pronounced differences between hits and misses enable threshold-based classification, the system noise during GPU inferences could significantly degrade classifier accuracy. In our experiments, we occasionally observed persistently elevated TTFT values over extended periods. These anomalies, due to their consistency over time, could not be addressed by merely excluding a percentage of outliers. To minimize such interference, we fully warmed up the GPU and introduced a sufficient pre-sampling delay. This approach allowed the system prompt to be reliably stored in the backend KV cache, stabilizing its acceleration effect for subsequent requests.
%We evaluated the classifier by randomly selecting 50 system prompts, sampling TTFTs for hit and miss conditions at a specific token length. The classification achieved a true positive rate (TPR) of 94.4\% and a true false rate (TFR) of 79\%. To improve classification precision, we will gather $n = 5$ time samples for each request, using $k = 3$ consistent outcomes as the decision threshold.  Additionally, a time discrimination range is defined; if more than 3 samples exceed this range, the samples are discarded, and re-sampling will be performed.
%\wenhao{here we evaluate the classification accuracy for a fixed token}
Using the profiled timing distributions for hits and misses, we are able to construct a simple classifier that determines a token as a hit if its latency falls below a predefined threshold. Importantly, as prompts grow longer, latency increases due to additional computational overhead. Additionally, the threshold must be calibrated based on the position of the token being recovered, as well as the specific hardware and model being targeted. Therefore, it is necessary to create $n$ classifiers, one for each of the $n$ tokens to be recovered. 

However, we observed that the TTFT can fluctuate due to factors such as GPU system noise and variations in voltage and power. These fluctuations reduce the effectiveness of using a fixed threshold as the classifier. To address this challenge, we propose a dynamic calibration scheme that adjusts the threshold in real time, improving the robustness of the classifiers. The core of this scheme is the simultaneous sampling of TTFT values that are guaranteed to miss the cache, within the same small time window during the measurement and recording of a given request’s TTFT. We then use these measurements to establish a baseline threshold, which represents the real-time performance of the serving system. Using this baseline, the threshold is dynamically adjusted during runtime.

To illustrate the classifier's accuracy, let us consider a specific example using the LLaMA-2-70B-GPTQ model under our evaluation settings. Consider we construct a classifier to determine whether the 10-th token hit the KV cache or not. Using the profiled timing distribution, we set the base threshold to 0.07971 seconds and dynamically adjust it based on the runtime state of the serving system. We evaluated the classifier's accuracy using 4,000 hits and 4,000 misses generated from randomly selected system prompts. According to our evaluation, the classifier achieved a true positive rate (TPR) of 0.76 and a false positive rate (FPR) of 0.02. To enhance the classifier’s robustness in prolonged and complex GPU usage scenarios, we employ $n=10$ sampling iterations. By defining a threshold $k=5$, a hit is determined when the observed hit count exceeds $k=5$, which improves the TPR to over 0.9.%\wenhao{do not emphasis theoretically}

%\link{I will redo the experiments in one day. My former method is kind of costly, the value of n and k will be determined withn 24 hours. The former result can be taken as the baseline.}
%\wenhao{update here if we use dynamic threshold}

%TPR: 0.7725
%FPR: 0.0000
\ignore{
\para{Recovering one token}
We previously explained how attackers preserve the system prompt in the KV cache. \autoref{fig:process_PSA} provides a detailed overview of the PSA attack process, focusing on recovering a single token of system prompt. During the offline phase, the attackers make two key preparations. First, they collect system prompts related to their target topic, ensuring semantic similarity, and fine-tune a language model to improve next-token prediction. Second, the attackers deploy a chatbot with a fixed system prompt in the KV cache and send user prompts to the SGLang backend, varying the shared prefix lengths with the system prompt. The returned TTFT variations are used to train a voting classifier, combining XGBoost, random forest, and gradient boosting, as simple thresholding is insufficient to handle system noise such as network latency and GPU load.

During the online phase, after the attackers employ statistical methods to obtain the system prompt’s initial tokens and verify them using TTFT, they send prompts to the fine-tuned language model to generate a probability distribution for the next token. Based on this distribution, the attackers randomly sample a candidate token, append it to the current prompt, and construct a new query. As \autoref{fig:distribution} shows, the prefill acceleration for a few tokens creates subtle and overlapping timing differences, increasing false positives when relying on single-sample evaluations. To address this, the attackers send up to $n$ identical requests to the SGLang backend which has the KV cache of the system prompt, records TTFTs. The voting classifier checks if the "Hit" count surpasses the threshold $k$; if so, the token is appended to the user prompt. Otherwise, the token's probability is penalized by halving the sampling probability to reduce the chance of incorrect predictions.

%\link{The process is given, now we need add more details of the dataset and model we've used. And show our experiment results.}



\textcolor{red}{We embedded over 350k diverse system prompts, 80\% of which are 500–1500 characters~\cite{systemprompt-huggingface}, using SBERT all-mpnet-base-v2~\cite{Send_request, reimers-2019-sentence-bert}. Then we calculated and extracted the largest cluster with cosine similarity over 0.9. From this, 200 prompts were randomly selected as the victim's system prompts, while the rest were provided to the attacker for fine-tuning. We fine-tuned LLaMa-3.1-8B-Instruct on an A100 GPU using LLAMA-Factory’s LoRA option~\cite{zheng2024llamafactory} for 20 epochs.}

%\link{Add how we can use evict \& flush methods here.}

\textcolor{red}{
The voting classifier relies on maintaining the system prompt's KV cache in the backend. Positive and negative samples are crafted with identical token lengths but differ in their shared prefix length with seperator and system prompt by $x$ tokens. Requests for both sample types are sent to the SGLang Chatbot system powered by the llama2-70B-GPTQ model, with their TTFT values recorded. TTFT differences between these samples guide classifier training, with 10,000 samples per category collected to avoid system noise. }




\link{We will use filter to eliminate some strange data, ensuring that these data are in a stable range. This can be categorized as challenge, please think about this question.}

\link{Optional tasks: warmup the GPU.}

\link{It seems we didn't have a closer look at the case that one-token hit and one-token miss, even we don't know why this amplify the performance, we can always predict for two tokens while recovering one single token. But this is not good, because we can't persuade the reviewers.}
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/PSA_Design.pdf}
    \caption{Process of PSA.}
    \label{fig:process_PSA}
\end{figure*}

\para{Building the classifier} 
In the \textit{offline phase}, we trained a cluster of classifiers, $classifier_0$ to $classifier_{n-1}$, where each $classifier_i$ ($0 \le i < n$) detects if the $i$-th token hits the cache, given that all preceding tokens have also hit the cache.

We used the llama2-70B-GPTQ model for evaluation. As shown in \autoref{fig:leakage_kv} (b), the timing difference between a cache hit and miss of 1 token is small (AUC=0.52), making it hard to build a robust classifier. Fortunately, we found that the timing difference can be enlarged by appending one dummy token right after the target token, i.e., adding the dummy token as the $i+1$-th token when building $classifier_i$. This may be because the dummy token takes up additional GPU computational resources, thus increasing the timing difference.


%timing difference between a cache hit and miss of 1 token is too negligible to be captured. However, we observe that the timing difference can be enlarged by appending one dummy token after the target token. This may occur because the dummy token occupies additional GPU computational resources, thereby increasing the timing difference. % Consequently, as long as there is at least one token that matches the shared prefix, we can detect the latency differences and potentially recover the token.

%To recover system prompt token-by-token, a cluster of classifiers is a must. For a fixed length, a classifier should be able to capture the nuanced timing differences after appending 1 more token as shared prefix. Specifically, $classifier_i $ ($0 \le i < n$) can detect whether the $i$-th token hits the cache. 

% In the \textit{offline phase}, we trained a cluster of classifiers, $classifier_0$, $classifier_1$, $\cdots$, and $classifier_{n-1}$, each capable of distinguishing between hit and miss cases for prompts of a specific length. Specifically, $classifier_i$ ($0 \le i < n$) is used to detect whether the $i$-th token hits the cache, conditioned on the fact that all previous tokens hit the cache. 

%The leakage above shows the negligible difference when the shared prefix is less than 2. Therefore, we choose shared prefix with 2 tokens as the goal of our classifier. 


% 这个地方不展示86,5的参数，应该只要展示一下0.55,0.42的TPR/FPR值就可以了

% @link, put it here
% the first paragraph outlines the goal of "Building the classifier" 
% the detail of the classifier follows

% OK.




%amplified by concatenating 1 random token after the target token. This is likely due to the random token consumes GPU's computation power, making the timing difference larger. As long as there is one or more tokens match with the shared prefix, we can detect the latency differences and subsequently recover a token.

%As shown in Figure~\ref{fig:histogram}\wenhao{@zixuan, the histogram here}\link{use the bar graph here to show the distribution},\wenhao{@link, fill in the text} as long as there is one or more tokens match with the shared prefix, we can detect the latency differences and subsequently recover a token.

\ignore{
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/histogram.pdf}
    \caption{Histogram for matching 0, 1, and 2 tokens when the lengths of the prompts are 2. The cases of matching 2 tokens (i.e., 2 shared) are distinguishable with other 2 cases.}
    \label{fig:histogram}
\end{figure}
% Histogram for cache hits and cache misses divided into row hits and row conflicts on the Ivy Bridge i5 test system. Measurements were performed after a short idle period to simulate non-overlapping accesses by victim and spy. From 180 to 216 cycles row hits occur, but no row conflicts
}

%\textcolor{red}{@Zixuan: Please add some details for the training model of classifiers here.}



We now describe the process of generating the dataset used to train $classifier_i$.
We first randomly sampled a system prompt $P$ from the dataset. We then generated 2000 unique sentences of length $i+1$ as negative samples, which all have the first $i-1$ tokens in common with $P$, but differ on the last two tokens. We also generated 2000 unique positive samples, which all have the first $i$ tokens in common with $P$ and a random dummy $(i+1)$-th token.
To collect the latency of the positive and negative samples, we first fed $P$ to the LLM server (SGLang with the llama2-70B-GPTQ model, then sent the sample to the LLM and measured the latency of each sample. Before collecting the latency of next sample, we flushed the KV cache to avoid noises.
%We choose sentences with one token longer prefix and dummy token at the end as positive samples. All positive and negative samples are of the same length.
%To train one classifier, we first initialize the LLM server (SGLang with the llama2-70B-GPTQ model in our experiment) with a random system prompt from our dataset.
% For the cache miss case, we generate 2,000 unique sentences. All these sentences have the same prefix and length, but they differ in the final two tokens. For the cache hit case, we use the same sentence length, but the prefix matches a segment of the system prompt. This ensures that the prefix is two tokens longer than the miss case, though the total sentence length remains the same.
%, and fed it to the LLM server (SGLang with the llama2-70B-GPTQ model in our experiment) for initialization
%Next, we send both sets of constructed samples to the LLM and measure the latency of each prompt. % In the hit case, because the prefix matches part of the system prompt, the LLM can use cached computations, leading to lower latency. In contrast, the miss case lacks this shared prefix, resulting in higher latency.
Based on the collected latency for both positive and negative samples, 
%we train a classifier to predict whether a given prompt has a matching prefix (hit) or not (miss). 
we utilized the XGBoost algorithm to train the classifier and optimized its hyper parameters using Bayesian optimization. To enhance the performance of the classifier, we adjusted the decision threshold to maximize the difference between the true positive rate (TPR) and false positive rate (FPR), while ensuring that the TPR remains high. In our evaluation, the classifiers have a TPR of 55\% and FPR of 42\%.
%Under the constraint of maintaining TPR, we set the point on the ROC curve of the trained classifier, where the difference between TPR and FPR is maximized
%\link{This might not be the truth, the maximized point of the difference between TPR and FPR is not good since at that point the FPR larger than 0.5, so we choose a relatively reasonable point.}, as the threshold for the classifier. 

% In our evaluation, the classifier achieves 80\% accuracy in recovering two tokens in a single attempt, while maintaining a false positive rate (FPR) below 10\%. Given the large search space for two tokens and the negligible latency difference between a hit on one token versus two tokens, we further evaluate the classifier’s precision on prompts with a shared first token. 

% We define a prompt as valid if, out of 50 trials, it results in a hit at least 25 times. The results show that for prompts sharing the first token, the true positive rate (TPR) reaches 86\%, while false positives are extremely rare, with an FPR below 5\%.%\wenhao{please make the text more concise (the reviewer needs to understand easily, without the need to guess unknown notations, such as what is shared first token, and one token hit two token hit (these are all grammar errors))}

%\wenhao{the above 2 paragraphs are unclear}

%\wenhao{@link: fill in the text}

%\link{Notes are shown below}

%\link{Changes the graph here a bit, False token => Two False tokens. Provide two versions for later selection.}
% data: 84 94 95, TPR => 90\% for similar sentences, FP case: barely found in similar and different sentences. 
% 










% classifier training sentences: Select the similar sentences or not. => The influence is only a little, so we can address it simply in one sentence. It is not so important.

}

\subsubsection{End-to-end attacks}
\label{subsubsec:psae2e}
%\hfill\\


\para{Vulnerable chatbot application}
We built a local chatbot using the FastChat framework as the victim application. It accepts the user's input and automatically concatenates it with a fixed system prompt to form the complete prompt which is send to the backend API server. The backend API server is built with SGLang v0.3.0.

In this evaluation, we used the \path{gabrielchua/system-prompt-leakage}~\cite{systemprompt-huggingface} dataset from Hugging Face, which contains over 350,000 synthetic system prompts. As outlined in \autoref{subsec:threat_model}, we assume the attacker has access to a public dataset of system prompts, and the victim's system prompts follow a similar distribution. To simulate this, we randomly selected 200 prompts from the dataset as the victim's prompts, while the remaining prompts were used by the attacker to fine-tune a model that predicts the next token based on recovered victim tokens.

\para{Attacks}
To mount the end-to-end attacks, we need to overcome several challenges.

\noindent\textit{$\bullet$ Timing measurement}.
As shown in \autoref{lst:time}, the attacker first sends a request to activate the system’s fixed system prompt. To ensure the corresponding KV cache is stably stored in the SGLang backend and optimally accelerates subsequent attack prompts, a brief delay is introduced after receiving the end-of-sequence marker from the POST response. Next, TTFT is measured by issuing a POST request with parameters set for a one-token maximum output. Timing starts with the request initiation and is recorded upon detecting the first non-blank token in the streamed response. %\autoref{lst:time} demonstrates how we measured the timing.%\wenhao{we should list the code snippet to get the timing measurement here}

\begin{figure}[htbp]
\centering
\begin{lstlisting}
def get_ttft(text):
    start_time = time.perf_counter()
    # Make sure in stream mode, max_token = 1
    response = requests.post({..., max_token=1,},
        stream = True
    )
    for line in response.iter_lines():
        if line:
            end_time = time.perf_counter()
            break
    ttft = end_time - start_time
    return ttft

def complete(text):
    # trigger the system prompt first.
    response = client.chat.completions.create(...)
    for line in response.iter_lines():
        if line:
            data = json.loads(line)
            if data.get("end_of_sequence", False):  
                end_time = time.perf_counter()
                break

# Wait for complete
complete(triggering_prompt) 
# brief delay for KV cache store.
time.sleep(0.2)
ttft = get_ttft(predicated_prompt)

\end{lstlisting}
\caption{Code snippet for measuring response time in KV cache side-channel attacks.}
\Description{}
\label{lst:time}
\end{figure}

\noindent\textit{$\bullet$ Flushing the caches}.
Since each request updates the KV cache and can affect subsequent TTFT measurements, the attacker must flush the KV cache after making the necessary queries to ensure accurate system prompt measurements. We observed that SGLang provides a $flush\_cache$ API~\cite{flush_cache} for efficient cache flushing. However, in our end-to-end attack, we chose not to use this API, as it is unlikely to be available to the attacker in real-world deployments. Instead, we employed a \textit{more robust method to evict the KV cache by sending irrelevant requests}. Using the default SGLang settings, a batch of 15 requests with approximately 500 tokens each was sufficient to trigger eviction. Each eviction took about 5 seconds on average and was successful 100\% of the time across 1,000 tests.



%\link{Below part is an optional part.}

%\noindent\textit{$\bullet$ Enhancing the robustness of classifiers}.

%\link{Here we emphasis on why we use multi-samples.}

%This approach significantly reduces the occurrence of false positives and false negatives, enhancing the reliability of the classification process.\wenhao{detailed steps with more concrete numbers are needed, e.g., why 10 and 30? how these numbers are set}

%0.95 for the \linewidth%
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/searchprefix_v3.pdf}
    \caption{Efficient token-by-token prompt recovery.}
    \Description{}
    \label{fig:searchprefix}
\end{figure}

\noindent\textit{$\bullet$ Token-by-token recovery}.
To reduce the search space, as shown in \autoref{fig:searchprefix}, in the \textit{online phase}, the targeted prompts are recovered token by token. %The process of recovering the next token involves several components: a \textit{next token predictor} that predicts the distribution of the next token based on the tokens already recovered, a \textit{sampler} that samples a candidate token according to this predicted distribution.
{The process uses a series of hit-or-miss \textit{classifiers} for validation and a \textit{next-token predictor} to estimate token probabilities, with a \textit{sampler} selecting candidates according to the predictor’s temperature setting.} For each candidate of the $i$-th token, the guessed prompt is fed into the LLM, to produce a set of TTFT values as the input of the $classifier_i$. The pre-trained classifier $classifier_i$ then evaluates the likelihood of the candidate token hitting the cache, indicating whether the token is correct. If it is deemed correct, the token will be appended to the prompt, and we continue to search for the next token. Otherwise, a \textit{repetition penalty} will be returned and applied to the probability corresponding to the current token to adjust the overall probability distribution.
Currently, we take a simple way to apply the repetition penalty, by halving the sampling probability of missed tokens in a new round.

%we've designed a prefix token predictor that can efficiently recover the secret system prompt. 
% The predictor mainly consists of two components, the classifier group and the token predictor. The classifier group is a group of different classifiers, each of them can classify the miss and hit cases of prompts of different length: for example, 
%the explain the flowo  of the figure (next token predictor, sampler etc.);

%The aim of our predictor is to infer the next token our input sentences using the timing differences of \textbf{Hit} and \textbf{Miss} cases. As demonstrated in Figure~\ref{fig:searchprefix}, the predictor mainly consists of the classifier group and the token predictor.

For constructing the next token predictor,
%On the other hand, the token predictor is the core of our system, 
%we assume the attacker has already obtain the several tokens of the system prompt using statistical forecasting methods since many system prompts start with common sentences like "You are a..". We also 
%For the prediction of the next token,
we used \path{LLaMA-3.1-8B-Instruct}~\cite{base_model} as the base model, fine-tuned with the training dataset available to the attacker. The model takes the partially recovered prompt and temperature as input, generating a probability distribution for the next token. The incorporation of temperature scaling introduces more randomness and diversity in token predictions. It's worth noting that our predictor is far from optimal as we used a single NVIDIA A100-PCIE GPU for LoRA fine-tuning, which only took about several hours. With improved fine-tuning settings -- such as a larger batch size, more epochs, or a bigger language model -- the performance of the predictor could be further enhanced.
%\textcolor{red}{more similar dataset}, 

%虽然检测1个token hit和miss的分类器的FPR很低（约0.02），但是如果在恢复某个token的过程中连续很多次next token predictor都给出错误的预测，则该token的FPR会累计，导致恢复出错误的token。

% As a solution, we concurrently issue requests without appended tokens and log their TTFT. We then compare these TTFT values to the predicted requests. If the TTFT difference exceeds the predetermined threshold time for token prefilling, we classify the current prediction as a failure.
%为了解决这个问题，我们通过在同一时间发送尚未加上新token的请求，记录TTFT并与预测的请求做时间对比。如果TTFT的相差值超过了一个token prefill所需时间的阈值，则我们判断本次预测失败。
% 明白了，可以丢到chatgpt，让它翻译成中文“请翻译为英文，使用学术语言：”
Although the FPR of the classifier in detecting a single token hit or miss is low (about 0.02, as shown in \autoref{subsubsec:chrctpsa}), the FPR for a token can accumulate during the recovery process if the next-token predictor repeatedly provides incorrect predictions. This accumulation can ultimately result in the recovery of an incorrect token. To resolve this, we introduce an additional cross-verification step for each candidate recovered token. Specifically, we send another query that does not append the token, which approximates the TTFT of a token hit. We then compare the TTFT value of this query to that of the predicted request. If the TTFT difference exceeds a predefined threshold for one-token pre-filling, we classify the current prediction as a failure, and proceed to the next guess. The token recovery process continues until either a preset number of tokens are correctly recovered or the maximum number of attack queries is reached.




%The attacker then continues attempting token recovery until



%Subsequently, the attacker proceeds to attempt token recovery until they have utilized the full predetermined number of allowable guesses.

%Via this method, the FPR can be reduced to xx.\link{update} 

%We input the sentence of the attacker and the given temperature to the model, the model generated the probability distribution of next token. 
%, and \textit{SGLang} as our LLM Server
%Based on the probability distribution, the sampler selects a new token, which is appended to the current prompt along with one dummy token. This new prompt is fed into the LLM to get the TTFT value.
%Same as the training process of the classifier, we initialize the LLM with a specific system prompt. 
%To obtain the new prompt, we append the new token to the former input. The new prompt will be fed into the LLM. In return, we will get the TTFT value.%\wenhao{more details}

%, generating a set of TTFT values. 
%explain experiment details: next token predictor (what base model, and fine-tuning is used), sampler (temperature scaling and how to adjusts the sampling probability), classifier  and explain the classifier (how $n$ and $k$ are determined)
\ignore{
To improve the classification accuracy, we need to collect a set of TTFT values for the classifier using the same candidate prompts in $n$ repetitive trials. For this purpose, we explicitly flush the cache and begin our timing measurements after the victim prompt is served in the LLM server.
%To flush the KV cache, we take advantage of SGLang's external APIs, i.e., \path{SGLang.srt.mem_cache.flush_cache} and the web API \path{http://SGLang-server:30000/flush_cache}.\footnote{Besides explicit API calls, alternative methods could also be used to flush the cache. Specifically,  the KV cache in SGLang adopts a simple LRU eviction policy that evicts the least recently used leaf first. Moreover, SGLang evict all cached tokens when the system receives a large batch size of requests. We leave the exploration in this direction as future work.}
%while others might need us to manually construct the eviction set based on the policy. 
We consider the candidate prompt to have hit the cache if the number of hits returned by the classifier exceeds $k$ out of $n$ trials. In our evaluation, we set $n = 100$ and $k = 50$, and the accuracy of correctly identifying a prefix cache hit is more than 86\%, and the FPR is about 5\%. %\wenhao{fill the text}
}


%可能还是一句话带过聚类，不然整个数据集有35万条数据，为什么非得选这1.6万条数据
%We further evaluated on the \textit{system-prompt-leakage }~\cite{systemprompt-huggingface} dataset, assuming the attacker is familiar with common expressions and vocabulary of system prompts. In particular, we semantically clustered the dataset to obtain over 16k distinct requests. From these, 200 were randomly selected as the test set, while the remaining requests were used for fine-tuning.\wenhao{we should not mention clustering; and why choose semantically clustering; or why clustering is reasonable? we cannot just say what we do, explain why it is reasonable to do it}

%With the next token predictor and the classifier above, we can recover the system prompt token by token, achieving an average accuracy of 92.3\% in recovering the tokens, with an average of 234 queries to the LLM to recover 1 token.

\para{Results}
%We randomly selected xx system prompts from the xx dataset, and used the above method to recover the prompts. 
We evaluated the recover accuracy, and the average number of attack queries required to recover every token. 
%We initially sought to recover the next token, given the first three tokens of the system prompt. 
% 2.642 * (10 + 10)
% 10 trails times and 10 threshold adjustment times.
Our findings reveal a recovery success rate of 86.5\%, with an average of 2.642 guesses and 52.83 attack queries to recover every token.  \autoref{tab:systemprompt} lists several examples of the correct system prompts, and part of the prompts recovered through the PSA.\wenhao{update data}


%Our findings reveal a recovery success rate of 86.5\%, with an average of 2.642 guesses and 52.83 attack queries per token and a 10.0\% FPR. The elevated FPR results from the predictor magnifying FP chances after unsuccessful predictions. To mitigate this, we contrast the TTFT of the token-appended request against the original. A TTFT delta exceeding a threshold signifies an incorrect prediction, necessitating token reversion and attack restart. Via this method, the FPR can be reduced to xx.\link{update} Subsequently, the attacker persists in attempting to recover the token until they have exhausted the predetermined number of guesses allotted to them. 
%\wenhao{please update}


% You act as a travel planning assistant specializing in personalized itineraries. Given a user's travel destination and preferences, provide a
% You act as

% You are a Travel Guide Assistant tasked with providing detailed travel itinerariesab a
% You are a 

%As a travel itinerary manager, you're tasked with crafting personalized travel options for users based on specific preferences and constraints. You must gather details on their interests, budget, preferred destinations, and travel durations to deliver tailored itineraries with suggested activities, accommodations, and dining options.

% As a vacation planner extraordinaire, you are tasked with creating personalized travel itineraries for clients. 
% 58 guesses
%We display only the first XX tokens that were recovered, along with the total number of attack queries.\wenhao{@link: fill in the number of recovered tokens}\link{The recovered tokens here is kind of different..}
\begin{table*}
    \centering
    \caption{Examples of recovered system prompts, along with the number of attack queries and recovered tokens.}
    \label{tab:systemprompt}
    {\small
    \begin{tabular}{C{0.5cm} | C{6.5cm} | C{6.5cm} | C{2.4cm}}
      \hline
   No. & Targeted system prompts & Recovered system prompts & \#queries/\#(recovered tokens)\\ \hline
   1 & You act as a travel planning assistant specializing in personalized itineraries. Given a user's travel destination and preferences, provide a multi-day itinerary $\cdots$ &  You act as a travel planning assistant specializing in personalized itineraries. Given a user's travel destination and preferences, provide a $\cdots$ & 1440/22 \\ \hline
   2 & You are an expert travel itinerary planner. Craft detailed and personalized travel plans for users based on their preferences and provided details $\cdots$ & You are an expert travel itinerary planner. Craft detailed and personalized travel plans for users based on their preferences and $\cdots$ & 1540/18 \\ \hline
   3 & Imagine you are a travel itinerary planner specializing in creating unique and personalized travel experiences. Your role is to craft itineraries that cater to the diverse interests and needs of travelers. These itineraries should $\cdots$ & Imagine you are a travel itinerary planner specializing in creating unique and personalized travel experiences. Your role is to craft itineraries that cater to the diverse interests and needs of travelers. $\cdots$ & 1080/34\\ \hline
    \end{tabular}
    }
\end{table*}

%\para{}
%\wenhao{Here, we lower the reviewer's expectations by admitting that in remote attacks, token by token recovery faces challenges.}
%\link{Describe the end-to-end scenario in this part. Draw a picture here.}
%\textcolor{red}{Following our analysis of side-channel leak risks from KV Cache sharing, we developed an end-to-end attack model to investigate system prompt leaks in real-world settings. Popular and representative chatbots like FastChat~\cite{zheng2023judging} improve model performance by positioning the system prompt, along with fixed fields of model chat templates that delineate its scope, at the forefront of the final composite prompt sent to the LLM.}
%Though time-based side channels from KV cache sharing are identified, leveraging them for valuable information is still uncertain. In our attack, we chose system prompts as our target. These prompts, which define the model’s configuration, can notably influence behavior with minor changes in wording~\cite{syspromptvalue}. Some prompts even boost performance, underlining their significant value~\cite{thinking-claude, zhang2024sprig}.



%(Guess we may need to select one of the sentence that can be hit, and repeat the lab for sufficient times.)
%explain how to flush the cache (there are 3 ways to flush the cache, we use the first one to demonstrate the attack)

% Need further the lab results.

% Two data are needed:
% 1. In the first round, what is the accuracy in 69 system prompts? TPR/FPR



% 老师，感觉这边的95%数字似乎是计算出来的，真实可能没有这么高？
% 或许说，theoritically
% 那能测一个真实的数字吗？只说理论值是不够的，reviewer关心真实值
% 数字应该没问题，但是样本可能不是那么多，可能只有69个
% 我这里的95%是一个token的准确率，不是整个prompt
% 对对对，我明白，这个我之前也大致算过
% 那最好有个实际统计的数字


%The results are shown in Figure~\ref{}.

% 我先撤了
% OK


\ignore{
for the system\_prompt dataset: 72 \%

Reason: Uncertainty of the tokenizer time for different token and different templates of sentences. So some 'different' senteces show a very bad result in prediction.

Defense: Diversity => against both the fine-tuned GPT predictor, and the Classifier. We can based on our case.
}
% AttentionStore only shares multi-turn dialog?

%\subsubsection{ChunkAttention}
%https://huggingface.co/papers/2402.15220

%In this paper, we introduce ChunkAttention, a prefix-aware self-attention module that can detect matching prompt prefixes across multiple requests and share their key/value tensors in memory at runtime to improve the memory utilization of KV cache. 

%Source code: %\url{https://github.com/microsoft/chunk-attention}


\subsection{Peeping Neighbor Attacks (PNA)}
%\link{Need great polishment. Too naive writting style.}
\label{subsec:evalpna}

\subsubsection{Attack overview}

%\hfill\\

In the PNA attack, we observe that not all user inputs contain sensitive information. For instance, an attacker is less likely to target inputs like "What’s the weather today?" Instead, the attacker focuses on specific, common queries that are more likely to contain private data. For example, an input such as "Draft a travel plan for my husband and me to Rome in September for a 3-day stay at the Hilton hotel" could reveal sensitive information, including personal data and location details. By identifying these high-risk queries, the attacker can exploit the timing side channel to retrieve data from a neighbor user's processed requests.

% Internet should be capitalized.
To identify such queries, we collected frequently asked, privacy-related questions from the Internet (\autoref{tab:templates}). Attackers seek to uncover associations between private attributes in these prompts, such as whether an individual is linked to a specific medical condition. The steps involved in the PNA attack are shown in \autoref{fig:semantic_attack}. 
Victim queries sent to the LLM are stored in a semantic cache, allowing the system to return cached responses for subsequent semantically similar queries. To exploit this behavior, attackers design queries containing private attributes and send them to the LLM while monitoring the TTFT. A significant reduction in TTFT, often below 1 second, indicates that the attacker’s query overlaps semantically with the victim’s prompts. This method enables attackers to confirm their hypotheses and gradually extract private information with high accuracy.

%After the victims send requests to the LLM, the serving system stores semantic caches of victim requests, reusing them for subsequent similar queries. Attackers prepare representative queries centered on their topic of interest and augmented with private attribute combinations. %When a victim submits similar queries, the attacker can attempt to extract private information by analyzing time differences in the semantic cache.
 %\wenhao{we should explain \autoref{fig:semantic_attack} in more details}
%Exploiting the semantic cache, which accelerates similar-query responses, attackers use TTFT measurements to validate their guesses, facilitating privacy leakage. 

%\autoref{tab:templates} lists a set of public templates that users might employ. 
In practice, users can convey the same meaning using different phrasing and may include different private attributes, such as personal names or medical conditions, in their queries. Our goal is to assess how these private attributes affect semantic similarity measures and to determine whether the resulting differences exceed the semantic threshold described in \autoref{subsec:pna_intro}. If they do, these differences could be detectable. This allows an attacker to infer private attributes by leveraging semantic similarity measures to distinguish between queries with or without an exact match of these attributes, even when victims use different phrasings.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/PNA.pdf}
    \caption{Peeping Neighbor Attacks}
    \Description{}
    \label{fig:semantic_attack}
\end{figure}



\begin{table*}
    \centering
    \caption{Examples of user prompts that contain private attributes.}
    \label{tab:templates}
    {\small
    \begin{tabular}{C{1.7cm} | C{15.2cm}}
      \hline
        \textbf{Use cases} & \textbf{Prompts} \\ \hline
       Healthcare  & Compose a meeting agenda for an interdisciplinary team discussing the treatment plan for \hl{[Name]} with \hl{[medical condition]}. \\ \hline
        Travel planning & I’m \hl{[flying/driving]} to \hl{[destination]} with \hl{[Name]} for a leisurely trip, and we’ll be staying at \hl{[hotel]} for \hl{[number of days]}. Can you create a comprehensive packing list organized by category?\\ \hline
        Business planning & Act as an expert business plan writer, and help me generate a product and services section of my \hl{[business type]} business plan. My company is \hl{[business]} called \hl{[business name]} that specializes in \hl{[USP or specialization]}. \\ \hline
        Performance review & I'm preparing for the annual performance review of an employee named \hl{[Name]}. \hl{[Name]}'s role involves \hl{[roles]}. Draft a performance review for \hl{[Name]} and suggesting improvements in \hl{[area of improvement]}. \\ \hline
        E-mails & Draft an e-mail to the \hl{[company]} on \hl{[subject]}. \\ \hline
        Cover letter & Write a conversational cover letter for \hl{[Name]} for a job application as a \hl{[position]} at \hl{[company]}. \\ \hline
        Out-of-office message & Write a short out-of-office message. Reason: \hl{[vacation]}. Dates: \hl{[month and dates]}. Person to contact in an emergency or for immediate help: \hl{[name]} at \hl{[email address]}. \\ \hline
    \end{tabular}
    }
\end{table*}

 


For this evaluation, we selected LangChain as the LLM serving framework due to its widespread adoption and extensive application ecosystem~\cite{Langchain-eco}. The local chatbot system was built on LangChain and integrated GPTCache~\cite{GPTCache_Usage} for semantic similarity-based request caching. 
The backend LLM was gpt-3.5-turbo in API mode, and we utilized the MedQuAD~\cite{MedQuAD-website} dataset for evaluation. 

%For this evaluation, we built a local chatbot system based on LangChain framework with GPTCache~\cite{GPTCache_Usage} to cache the requests based on semantic similarity.

\ignore{
\textcolor{red}{
We used the albert-base-v2~\cite{onnx_albert} model in ONNX~\cite{onnx-github} to compute semantic similarity, striking a balance between accuracy and efficiency for robust prompt analysis. While the default SearchDistanceEvaluation ~\cite{searchdistance} method is faster and maintains attack efficacy, it is more likely to misclassify unrelated sentences as similar, leading to irrelevant responses that could compromise the system’s usability.}
}

\subsubsection{Characterizing the leakage}

%\hfill\\





%h!
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth]{figures/semantic_leakage.pdf}
    \caption{Semantic leakage of privacy attributes.}
    \Description{}
    \label{fig:Semantic}
\end{figure*}

%\link{Since Medical is not a noun, change value name here.}

The evaluation steps are shown in \autoref{fig:Semantic}. %We took a specific template ``Compose a meeting agenda ... for \hl{[Name]} with \hl{[medical condition]}.'', denoted by $T_0$ as an example. In this case, both name and medical condition are private attributes of the patient.
We employed the template "Compose a meeting agenda ... for \hl{[Name]} with \hl{[medical condition]}," denoted as $T_0$ as an example, where both the name and medical condition are private attributes of the patient.
In the \textit{first} step, we randomly sampled 10 $Names$ from the python package \path{names-dataset}~\cite{NameDataset2021} and obtained 10 random 
medical conditions by sampling 10 semantically unrelated Q\&A pairs from the MedQuAD dataset, extracting the $Medconds$ using GPT-3.5-turbo.
%. To obtain 10 random medical conditions, we randomly sampled 10 semantically unrelated Q\&A pairs from MedQuAD dataset and used \path{gpt-3.5-turbo} to summarize the medical conditions from questions. We randomly sampled 1 name and 1 medical condition, denoted by $Name_0$ and $Medcond_0$, as the private attributes to be recovered, while the other pairs are used to generate negative group (described in the next paragraph).


In the \textit{second} step, to address variations in how victims might express the same semantics, we generated sentences semantically aligned with the template $T_0$. GPT-3.5-turbo was used to paraphrase $T_0$, % using \path{gpt-3.5-turbo} and generated
producing $n$ semantically similar sentences $\{T_1,..,T_n\}$ with $Name_0$ and $Medcond_0$ filled in the template. %\textcolor{red}{Sentences with semantic similarity scores below a predefined threshold were excluded.}

After completing the two previous steps, we generated two sample groups: the positive group, which includes templates filled with
%After the above two steps, we've generated two groups of samples: the positive group consists of all generated templates filled with 
$Name_0$ and $Medcond_0$, i.e., $\{(T_i, Name_0, Medcond_0) | i = 1, \cdots, n\}$; the negative set, which consists of the original template filled with other names or medical conditions, i.e., $\{(T_0, Name_i, Medcond_j) | i \ne 0~or~j \ne 0\}$. 
Moreover, we split the positive group into two subsets: the first one (20\%) is used as positive samples, and the rest are used as evaluation group. We made sure the positive group and negative group are of the same size.

%In the last step, we computed the semantic similarity between the evaluation cases and the positive group, as well as between the evaluation cases and the negative group. This process yields the respective similarity vectors of the positive and negative groups. 

In the final step, we computed the semantic similarity between the evaluation cases and both the positive and negative groups, generating the respective similarity vectors.

When semantic similarity exceeds a predefined threshold, it can trigger observable acceleration, increasing the risk of misclassifying negative samples as positive. To address this, we introduced the ROC curve to evaluate possibility of this risk. %, which visualizes the tradeoff between the false positive rate (FPR) and true positive rate (TPR) and is commonly used to evaluate classifier performance. 
By analyzing the ROC curve, we can determine whether semantic leakage, induced by privacy attributes, is both detectable and exploitable.

We assessed semantic differences across thresholds from 0.6 to 0.9, with the default value in GPTCache set to 0.8. The ROC curves in \autoref{fig:semantic_roc} illustrate the clear distinction between the positive and negative groups. For instance, at the default threshold of 0.8, a TPR of approximately 0.95 corresponds to an FPR of less than 0.1.

Additionally, we explored cases where only one private attribute matched. In this scenario, the negative group consists of sentences with a single correct private attribute, while the positive group remains unchanged. As shown in  \autoref{fig:semanticone_roc}, the semantic differences between the groups remain substantial. For example, with the default threshold of 0.8, a TPR near 0.85 still results in an FPR below 0.1.

%\textcolor{red}{Semantic similarity can cause observable acceleration once it exceeds the predefined threshold, which introduces the potential for negative samples to be incorrectly classified as positive if their similarity surpasses this threshold. To address this, we integrate the ROC curve into the binary classification model.}

%\textcolor{red}{The ROC curve, which visualizes the tradeoff between the false positive rate(FPR) and the true positive rate(TPR), is a standard method for assessing classifier performance. By analyzing the ROC curve, we can evaluate whether semantic leakage, arising from privacy attributes, is both detectable and exploitable.}

% \begin{figure*}
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/two_curve.pdf}
%         \caption{The ``name'' and ``medical condition'' in the negative group are both different from the positive group.}
%         \label{fig:semantic_roc}
%     \end{subfigure}
%     \hspace{15pt}
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/sin_curve.pdf}
%         \caption{Either the ``name'' or ``medical condition'' in the negative group is different from the positive group.}
%         \label{fig:semanticone_roc}
%     \end{subfigure}
%     \caption{Leakage profile of sharing the semantic cache. We plotted the ROC curve to fingerprint the timing difference between the similarity vectors of the positive and negative groups.}
%     \label{fig:semanticsim}
%     % Maybe add another graph here.
%     % WE've only studied the 'name' case.
% \end{figure*}

\begin{figure}[!ht]
    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/two_curve.pdf}
        \caption{The ``name'' and ``medical condition'' in the negative group are both different from the positive group.}
        \label{fig:semantic_roc}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sin_curve.pdf}
        \caption{Either the ``name'' or ``medical condition'' in the negative group is different from the positive group.}
        \label{fig:semanticone_roc}
    \end{subfigure}
    \caption{Leakage profile of sharing the semantic cache. We plotted the ROC curve to fingerprint the timing difference between the similarity vectors of the positive and negative groups.}
    \Description{}
    \label{fig:semanticsim}
\end{figure}

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=.95\linewidth]{figures/semanticsim.png}
% \caption{Leakage profile of sharing the semantic cache. We plotted the ROC curve to fingerprint the timing difference between the similarity vectors of the positive and negative groups.\link{Use a smaller graph, changed the curve markers to make it clearer for classifications.}}
% \label{fig:semanticsim}
% \end{figure*}

%We evaluated the semantic differences under different semantic thresholds ranged from 0.6 to 0.9 (the default value in GPTCache is 0.8), and the ROC curves between the similarity vectors of the positive and negative groups are shown in \autoref{fig:semanticsim} (a). It can be seen that the positive and negative group can be well distinguished. For example, in the default setting (threshold = 0.8), when the TPR is close to 0.95, the FPR is still less than 0.1.

%Besides, we further evaluated the effect of the cases when only 1 private attribute matches. For this purpose, the negative group consists of sentences with only one correct private attribute using the same template, while the positive group remains unchanged. The result (\autoref{fig:semanticsim} (b)) shows  that the semantic differences between the positive group and negative group are still large enough. For example, in the default setting (threshold = 0.8), when the TPR is close to 0.85, the FPR is still less than 0.1.


%Simultaneously, to prevent the negative influence of incomplete private attributesrmation leakage on our attempts to restore full privacy, we conduct another experiment to distinguish between individual privacy factors and complete privacy factors. Concisely, the negative group involves sentences with only one right privacy factor using the same template, while the positive group remains unchanged. Results in ~\ref{fig:semanticone_roc} indicates significant semantic differences between complete and incomplete private attributesrmation groups. For instance, in the default setting (threshold = 0.8), when the true positive rate (TPR) is close to 0.85, the false positive rate (FPR) is still less than 0.1.

%The result demonstrated in Figure~\ref{fig:semantic_roc} indicates a relatively low False Positive Rates(FPR) in all of our test suites. When the True Positive Rate(TPR) is close to 0.95, the FPR is still lower than 0.1. Notably, when we choose 0.8 as the threshold, we have best performance in separating HIT/MISS cases.

% \link{graphs here should be changed later.}


%seeds and the samples, and obtain the similarity matrix at the end. In order to enhance the generalizability of the results and increase the sample size, we conducted the experiment 50 times and plotted ROC curves based on the relevant data.


%in semantic similar sentences "seeds". We randomly choose 80\% as our positive samples, the remaining 20\% as our evaluation data.

%Following are our steps shown in Figure~\ref{fig:Semantic}:

%The adversary is interested in recovering the private attribute about a target individual, given its name and corresponding domain knowledge.

%We design an experiment to fulfill our idea that the semantic differences introduced from private attribute are significant enough to be recognized. For example, assume we want to develop a treatment plan for \textbf{\{Name\}} with \textbf{\{Medical Condition\}} using LLM. In this scenario, both the name and medical condition are privacy to the patient. Following are our steps shown in Figure~\ref{fig:Semantic}:

\ignore{
\begin{itemize}
    \item First, we select a template $T_0$ to be filled in later.
    \item Second, we select 10 different Names from the \textit{NameDataset} package in python. And randomly select 10 semantic unrelated Q\&A pairs from the dataset. Besides, we use \path{gpt-3.5-turbo} to summarize the medical condition from the question. We then choose $Name_0$ and $Medical_0$ as our privacy, and form the seed $(T_0, Name_0, Medical_0)$, while other pairs will be stored in keywords.
    \item Third, to obtain the template cluster, we paraphrase the template ($T_0$) without changing the keywords using \path{gpt-3.5-turbo}. After filling in new template $\{T_1,..,T_n\}$ with $Name_0$ and $Medical_0$, we utilize the threshold of GPTcache to filter in semantic similar sentences "seeds". We randomly choose 80\% as our positive samples, the remaining 20\% as our evaluation data.
    \item Next, we use the original template $T_0$, fill in with different names and medical conditions as the negative samples. The number of the negative samples equals to the positive samples, and can be represented as $NS$, which is the subset of $\{(T_0, Name_i, Medical_j)|i \neq 0 \lor j \neq 0\}$.
    \item Finally, using the same threshold, we calculate the similarity between our seeds and the samples, and obtain the similarity matrix at the end. In order to enhance the generalizability of the results and increase the sample size, we conducted the experiment 50 times and plotted ROC curves based on the relevant data.
\end{itemize}
}


%1. how you build your chatbot system


%2. what model is used, what dataset is used

%3. query from different session or different users, how it is tested

\subsubsection{End-to-end attacks}

%\hfill\\

%\textcolor{red}{@Linke: given our crafted dataset, the accuracy under typical threshold}

\para{Victim queries}
%\wenhao{it seems that we are missing a type: how many queries of both the name and medical condition match; we also need to specify the process of end-to-end attacks, i.e., how we the experiments are conducted: the victim sends 4 types of requests in random order (e.g., in total 40 negative queries and 10 true positive groups), and the attacker conduct 1 round of attacks, and count how many FPR/TPR}
We consider a typical open-world scenario where a victim user queries the LLM for healthcare assistance, using the template ``compose a meeting agenda ..'' from  \autoref{tab:templates}. In practice the user may customize the template with different names and medical conditions. Additionally, the user might ask questions unrelated to the template. To simulate this, we model the user making the following four types of queries:

\begin{packeditemize}
    \item Type-1 (true samples): queries with the name ``Alice'' and with specific medical condition like ``heart disease''.
    \item Type-2 (false samples): queries with the name ``Alice'' but with differing medical conditions such as ``diabetes'', ``hypertension'', and ``asthma''. 
    \item Type-3 (false samples): queries with the medical condition ``heart disease'', but with different name.
    \item Type-4 (false samples): unrelated queries with different names and different medical conditions. 
\end{packeditemize}

We assume that the attacker targets the private attribute associations found in Type-1 requests. The victim is simulated to choose passphrases freely, while preserving the same meaning. We hypothesize that the victim sends requests randomly, with each round consisting of five requests: 1 true sample as a Type-1 request and four false samples, including 1 Type-2 request, 1 Type-3 request, and 2 Type-4 requests. The attacker conducts attacks on each of the victim’s requests. %It is assumed that the binding relationship between two private attributes of Type-1 requests aligns with the attacker’s aim to confirm this specific association. 
We use the TPR to evaluate the effectiveness of recovering these private attributes in true samples, and use separate FPRs to measure the error rates of incorrectly classifying the 3 types of false samples as positive.

%type to capture errors.

\para{Eviction}
%Frequent victim requests\wenhao{why victim requests; we need to flush attacker's request?} to GPTCache can cause sensitive information to overlap with unrelated data, hindering the identification of specific relationships, such as a name associated with a disease. Therefore, eviction on GPTCache is required for end-to-end attacks.
%Our experiments show that sending more semantically unrelated requests than the cache’s capacity (default: 1000) triggers the cache replacement policy (default: LRU) to evict existing entries, releasing space proportional to the \textit{clean\_size}~\cite{clean_size} parameter in GPTCache.
%\wenhao{In my understanding, this does not specify how to evict the targeted cached data?? The reviewer does not care about cleansize: send 1000 unrelated requests to evict only a small portion of cached entries?? then how to evict the target entry: send 1/cleansize * 1000 unrelated requests??}
%Successful end-to-end attacks on the semantic cache
%LLM serving system 
%requires eliminating the
%depend on addressing 
%interference from residual attacker inputs in the semantic cache,
To perform end-to-end attacks on the semantic cache, we must eliminate any interference caused by the attacker's own requests, as these also reside within the semantic cache.
%especially \textcolor{red}{as targeted private attributes differ in each round}\wenhao{maybe we do not need to explain this}. \link{Make sense}
To address this, we developed a method to evict all of the attacker's requests from the semantic cache after each round of attack trials. Specifically, our experiments show that, with the default configuration of GPTCache, sending 1,000 semantically unrelated requests is sufficient to remove the residual entries from the cache.
%Eviction from GPTCache is essential in this context. 
%Our experiments show that, with the default configuration of GPTCache, sending 1,000 semantically unrelated requests is enough to evict all residual entries from the semantic cache.
%Our experiments indicate that under the default configuration of GPTCache, sending 1000 semantic unrelated requests is sufficient to evict all residual entries in the semantic cache. %\wenhao{why use "if not", and "the desired evicted entries" is not important, we need to evict the specific entry, so we need to send the same number as the cache size?} %The eviction queries are purposefully unrelated to the attacker’s target topics, and their high semantic diversity ensures a more thorough clearing of undesired cache content.
%clearing existing entries. %and freeing space determined by the \textit{clean_size} parameter~\cite{clean_size}. 
%These eviction queries are not related to the attacker’s targeted topics, and greater semantic dissimilarity among them enhances the effectiveness of the eviction process.

\para{Attacks}
The attacker aims to determine whether a specific user ``Alice'' is associated with a particular medical condition, such as ``heart disease''. Since the victim may use various passphrases, the attacker sends multiple queries to improve coverage and achieve a higher TPR. However, sending additional queries can also increase the likelihood of false positives (i.e., a higher FPR) if these new prompts closely resemble earlier ones. To address this challenge, he prioritizes \textit{representative queries} in the attacker's query space and increases the volume of queries while minimizing mutual interference.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/semantic_challenge.pdf}
%     \caption{Challenges of PNA.}
%     \label{fig:semantic_chanllenge}
% \end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/semantic_space.pdf}
    \caption{The greedy searching strategy for PNA.}
    \Description{}
    \label{fig:semantic_space}
\end{figure}

%\link{Draw a new graph here, emphasis on the threat model we use, extend section 2.4.}

%\wenhao{missing important end-to-end attack information here: what is the victim query (how many non-relevant queries are made, how are the relevant, i.e., hit the template, queries like), how the attack uses the generated candidates to infer the victim query, i.e., exact matching the two private attributes, how the FPR/TPR are calculated}

%In real-world PNA attacks, there may be overlaps in the search space. As a result, the attacker might need to send multiple queries to improve coverage and achieve a higher TPR. However, sending additional queries can also increase the likelihood of false positives (i.e., a higher FPR) if these new prompts closely resemble earlier ones. To address this challenge, we prioritize \textit{representative queries} in the attacker's query space and increase the volume of queries while minimizing mutual interference.

%To address these challenges, there are two main strategies for selecting attack prompts: selecting the requests that are \textit{most representative} of the attack space; and increasing the number of attack attempts.

%We define the \textit{most representative} requests as those that are nearest to other requests in the sentence space with the same semantics. Specifically, we use \textit{distilbert-base-uncased} as the model to obtain the embeddings of all sentences in the sentence space and employ euclidean normalization methods to sort the requests by L2 distances from low to high. Therefore, the smaller the index of a sentence within the group, the more representative it is for the entire sentence space. After sorting, we can use sentences with smaller indexes as attack prompts to increase the coverage of the attack.

\textit{Representative} queries are defined as those closest to others in the semantic space. Using distilbert-base-uncased model, we generate embeddings and sort queries by L2 distance. Queries with the smallest indexes are deemed most representative and selected as attack prompts to maximize coverage.
Expanding coverage necessitates issuing additional \textit{orthogonal prompts}, which are semantically distinct from one another. This approach ensures that semantic overlaps among the attacker’s prompts do not compromise the accuracy of identifying victim responses. 
Given the low FPR shown in \autoref{fig:semanticsim}, any cache hit can indicate semantic overlap. While this improves coverage, it also raises FPR, demanding careful trade-offs.

%As shown in \autoref{fig:semantic_space}, we designed a greedy searching algorithm that aims to find the \textit{most representative} requests for a target sentence. Specifically, suppose that the target space (a subspace of the whole space, denoted by shaded area) is the sentences that are judged as semantically similar with the target sentence, then the attack goal is to expand the coverage within the target space by sending orthogonal prompts.

Building on the two proposed tactics, \autoref{fig:semantic_space} presents our greedy search strategy for identifying the \textit{most representative} requests within a semantically similar target space, thus improving the accuracy of PNA.
Specifically, at each iteration, the algorithm selects the most representative candidate (e.g., $\alpha$) and adds it to the attack set unless it is too similar to existing members (e.g., $\beta$). The process halts when no candidates remain or when the FPR exceeds a preset threshold $\sigma$. %\textcolor{red}{$\sigma$ is a composite parameter derived from analyzing TPR, FPR, and trails, optimized through a systematic machine learning process. This parameter enables attackers to effectively balance these variables, achieving an expanded attack range while maintaining high accuracy at minimal cost.}\wenhao{the last sentence is vague. Make it clear or remove it. Try to avoid this type of sentence throughout the paper.} \link{Do we need to provide the concrete method to get $\sigma$'s value? I don't think it necessary.}


%in every searching step, we always select the one in the sentence space that is most representative in the remaining candidate set (e.g., $\alpha$) and add it into the attack set. If the most representative one (e.g, $\beta$) is too close to any member of the attack set, we skip it and continue to search for the next one. 
%The process stops if any of the following conditions is met: there are no remaining candidates in the sentence space, or the FPR exceeds a preset number $\sigma$.


%we can also attack in more trials. Nevertheless, the similarity between attack attempts themselves might introduce noise in the semantic cache system. Thus, to mitigate this interference, we should always select orthogonal sentences as attack prompts.

%Based on the two insights above, our attack focuses on increasing the number of \textit{most representative} attempts. The strategy is demonstrated in Figure~\ref{fig:semantic_space}. The target is a part of sample spaces that are similar to the original target. The red points are attack candidates. We always select candidates based on their levels of representativeness, from highest to lowest. After sorting, assume the \textit{most representative} point is $\alpha$, it can cover a range of semantic neighbors. If the target has a sentence of semantically close and paraphrased form of $\alpha$, it will be detected. In order, we should select $\beta$, which covers great amount of target. However, $\beta$ are not orthogonal, or too close to $\alpha$. Therefore, selecting $\beta$ as attempt will hit with $\alpha$, causing unexpected false positive cases. What we can select is $\gamma$, though it only covers little amount of target, it is orthogonal to $\alpha$.

% We choose 
\ignore{
% We consider hit if at least attack 
According to \autoref{fig:semantic_space}, while selecting more prompts can increase coverage, it does not guarantee improved accuracy. Thus, we select several parameters to judge whether we should halt or continue our experiment.
\begin{itemize}
    \item $\Delta TPR$ and $\Delta FPR$: represent the change of true positive rates and false positive rates after selecting one more attack candidate.
    \item $\Delta Times$: represent the increment of test times after selecting one more attack candidate.
\end{itemize}
}
% We set a hyper parameter $\chi$ controlled by the attack to evaluate whether we reach the halting conditions or not, with the following formula. 

% $$\chi = \frac{0.4 \cdot exp(\Delta TPR) - 1.0 \cdot \Delta FPR }{1 + 0.5 \cdot \sqrt{\Delta Times}}$$

%  We calculate the value of $\chi$, if the value if below 0.4 ()

\para{Results}
%\link{https://gptcache.readthedocs.io/en/latest/usage.html?highlight=evict}
In the evaluation, we repeated the experiment 500 times for each of the 4 types of victim queries. In every iteration, a randomly pair of private attributes in Type-1 request is chosen. %\wenhao{maybe 4 types}
%both the positive and negative samples (derived the same way in \autoref{fig:Semantic}) contained 695 sentences.
We found when we set the threshold $\sigma$ to 0.04, the attackers can achieve an expanded attack range while maintaining high accuracy at minimal cost. In this condition, we identified at most 5 \textit{orthogonal} attack prompts with the proposed greedy search strategy. \autoref{tab:semantic_attack} shows the TPR of true samples, and seperated FPR for each type of false samples as %the number of attack prompts 
trails increases from 1 to 5. %In particular, the attack can achieve a 85.3\% TPR and 3.2\% FPR with only 2 trials, while the attack can achieve approximate 90\% TPR and 3.9\% FPR with 5 trials. \wenhao{unify the use of \% or not}
%\wenhao{maybe we should give some insight based on the results here, which may be filled in later}\link{OK. Maybe I need to first ensure the data here.}\link{The Type2 data is kinda strange,}\link{Fixed.}
% [0, 411, 41, 8, 7, 3, 1, 1, 0, 3, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0] 500
%[0, 311, 69, 39, 17, 11, 1, 2, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0] 500
%tpr: 
%     82.2%  62.2%
%     90.4%  76.0%
%     92.0%  83.8%
%     93.4%  87.2%
%     94.0%  89.4%
%fpr:
%
%
%
%
%

% fpr: 0.031654676258992806 tpr: 0.8532374100719424  fpr_test_time: 695 tpr_test_time: 695 
% maximum select 2 sentences
% fpr: 0.033093525179856115 tpr: 0.9194244604316547  fpr_test_time: 1207 tpr_test_time: 788 
% maximum select 3 sentences
% fpr: 0.03597122302158273 tpr: 0.9510791366906475  fpr_test_time: 1553 tpr_test_time: 829 
% maximum select 4 sentences
% fpr: 0.03884892086330935 tpr: 0.962589928057554  fpr_test_time: 1786 tpr_test_time: 843 
% maximum select 5 sentences
% fpr: 0.03884892086330935 tpr: 0.962589928057554  fpr_test_time: 1899 tpr_test_time: 848 
% maximum select 6 sentences
% fpr: 0.03884892086330935 tpr: 0.9640287769784173  fpr_test_time: 1975 tpr_test_time: 850 
% maximum select 7 sentences
% fpr: 0.03884892086330935 tpr: 0.9640287769784173  fpr_test_time: 2013 tpr_test_time: 850 
% maximum select 8 sentences
% fpr: 0.03884892086330935 tpr: 0.9640287769784173  fpr_test_time: 2037 tpr_test_time: 850 
% maximum select 9 sentences
% fpr: 0.03884892086330935 tpr: 0.9640287769784173  fpr_test_time: 2048 tpr_test_time: 850

% Compose a meeting agenda for an interdisciplinary team discussing the treatment plan for Alice with heart disease.

%     82.2%  62.2%
%     90.4%  76.0%
%     92.0%  83.8%
%     93.4%  87.2%
%     94.0%  89.4%

%[0, 58, 13, 2, 2, 1, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0]
%[0, 343, 71, 37, 21, 12, 7, 6, 2, 1, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0]
%[0, 27, 2, 3, 3, 3, 1, 1, 1, 1, 0, 0, 0, 0, 0, 0, 0, 0, 0, 0] 500
\begin{table}[!th]
 \centering
    \caption{Attack accuracy for the 4 types of victim queries with different number of attack trails.}
    \label{tab:semantic_attack}
     {\small
    \begin{tabular}{C{1.0 cm} | C{1.0 cm}| C{1.0  cm} | C{1.0  cm} | C{1.0  cm} }
    \hline 
         \textbf{\#Trials}    & \textbf{Type 1 \newline (TPR)} & \textbf{Type 2 \newline (FPR)} & \textbf{ Type 3 \newline (FPR)} & \textbf{ Type 3 \newline (FPR)} \\ \hline  % & Automatic sharing 
        1 & 0.814 & 0.116 & 0.054 & 0.004\\ \hline
        2 & 0.884 & 0.142 & 0.056 & 0.005\\ \hline
        3 & 0.930 & 0.146 & 0.060 & 0.005\\ \hline
        4 & 0.946 & 0.150 & 0.062 & 0.005\\ \hline
        5 & 0.954 & 0.152 & 0.062 & 0.005\\ \hline

    \end{tabular}
    }
\end{table}


%\subsubsection{KV cache sharing in RAG}
%\subsection{Timing Attacks on RAG}
\subsection{Inferring Processed Documents with KV-cache Side Channels on Commodity Models}
\label{subsec:psarag}

% In this section, we present an end-to-end demonstration of the potential vulnerabilities associated with KV-cache side channels in real world LLM API services. Specifically, we examine an application using the GPT4o mini model to tag and caption images, following OpenAI's guidelines~\cite{openaiimagecaption}. Our experimental setup highlights how an adversary could infer processed documents by analyzing timing side channels associated with the KV cache.

% In this scenario, user-provided images are submitted as part of messages under the ``user'' role. These messages are sent to OpenAI's backend model, which generates image descriptions and captions. Importantly, all user inputs are processed under a single shared API account, a common setup for such applications. Furthermore, since OpenAI's API supports prompt caching~\cite{promptcachingopenai}, cached data may be inadvertently shared among different users of the application, raising significant privacy concerns. This issue becomes especially critical when sensitive information is involved, as attackers could exploit timing side channels to infer the inputs of other users.

% To evaluate this vulnerability, we developed an image captioning application strictly following OpenAI's guidelines~\cite{openaiimagecaption}. In our experiment, we assume that an attacker is interested in determining whether a victim has submitted a specific image for captioning. The attacker prepares a set of 10 interested images and periodically queries the application. Meanwhile, the victim is simulated to submit one image from the interested set and one random image outside of it. This process is repeated 10 times for the 10 interested images, and we record the attack's success rate in correctly identifying the victim's image.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/response_times.pdf}
    \caption{Timing distribution for hits and misses of processed documents with 12,000, 18,000, and 24,000 tokens.}
    \Description{}
    \label{fig:infer_documents}
\end{figure}

In this section, we present an end-to-end demonstration of the potential vulnerabilities associated with KV-cache side channels in real world LLM API services. Our experimental setup highlights how an adversary could infer processed documents by analyzing timing side channels associated with the KV cache.

\para{Vulnerable application}
Specifically, we examine an application using the Deepseek-chat model to analyze PDF documents, following guidelines outlined in Deepseek's documentation~\cite{deepseekguide}. The application begins by converting user-uploaded PDF files into text using the \path{pdfplumber} package, which extracts the textual content from each page of the PDF. The resulting text is then formatted into a request and sent to the LLM backend for processing and summarization.
In this scenario, user-provided documents are included in messages under the ``user'' role. These messages are sent to Deepseek's backend model, which generates document summaries. Notably, all user inputs are handled through a single shared API account—a typical configuration for such applications. However, this setup introduces privacy risks due to Deepseek's support for prompt caching~\cite{promptcachingopenai}, cached data may be inadvertently shared among different users of the application, raising significant privacy concerns. This concern becomes particularly serious when sensitive information is involved, as a malicious user could exploit timing side channels to infer the processed documents of other users.

%To evaluate this vulnerability, we developed a PDF document summary application strictly following  Deepseek's guidelines~\cite{deepseekguide}. 
\para{Characterizing the leakage}
We extracted 200 documents with varying lengths of approximately 12,000, 18,000, and 24,000 tokens, saved in PDF format, by segmenting the long-text zero\_scrolls dataset~\cite{shaham2023zeroscrolls}. Our evaluation revealed distinct latency patterns for cache hits (repeatedly sending cached documents) and cache misses (sending uncached documents), as illustrated in \autoref{fig:infer_documents}. Specifically, the response times for cache hits were consistently distributed within the same range across documents of different lengths. In contrast, the response times for cache misses increased as the document length grew.

\para{End-to-end attacks}
In this evaluation, we assume that an attacker is interested in determining whether a victim has submitted a specific document for summarizing. The attacker prepares a set of 200 interested documents and periodically queries the application. Meanwhile, the victim is simulated to submit 100 documents from the interested set and other 100 random documents outside of them. This process is repeated 5 times for the 100 interested documents, and we record the attack's success rate in correctly identifying the victim's document.

Specifically, we conducted experiments using documents of varying lengths ranging from 12,000 to 24,000 tokens. The victim initially submitted 100 target documents of mixed lengths to the system. The attacker then performed a single probing attempt on each of these 100 target documents, recording the response times. Using these results and a predefined threshold of 2.0 seconds, we computed the TPR as the proportion of target documents correctly identified as hits (response times below the threshold). Subsequently, the victim submitted 100 non-target documents of mixed lengths, and the attacker again attempted to probe using the target documents. The FPR was calculated as the proportion of non-target documents mistakenly identified as target documents based on response times below the threshold. The experimental results demonstrated a TPR of 0.89 and an FPR of 0.05.

\para{Notes}
For ethical reasons, we chose not to explore methods for efficient cache eviction in real-world serving systems, as this would require extensive experiments that could potentially violate system policies or negatively impact user experience. Without proactive cache eviction, the granularity of the attack is limited to the point when cached content is removed due to inactivity -- typically around 5 minutes in systems like OpenAI and Anthropic, as noted in their documentation~\cite{promptcachingopenai,claudepromptcaching}.

%However, we believe that cache eviction is still possible, given that cache space is limited, which is also supported by our evaluation in the local SGLang setup (\autoref{subsubsec:psae2e}).

%\wenhao{@zixuan: results here}


%please see the comment
% https://mp.weixin.qq.com/s/PjMyqWftpvX5mebbnrMVwA
% 搜索改写查询文档并且将其向量化以后,甚至是计算中的KV Cache都可以缓存到一些内存数据库, 当下一个用户问相关问题的时候,然后利用SplitWise的方式, 直接可以把这些KV Cache进行Prefill了. 另外还可以把这些Prompt Summary以后做Cache等. 这也是通常数据层面中采用RAG/Prompt Summary的方式, 

%\subsubsection{RAGCache: Efficient Knowledge Caching for Retrieval-Augmented Generation}

%https://arxiv.org/abs/2404.12457

% First, the recurrence of identical documents across multiple
% requests enables the sharing of LLM inference’s intermediate
% states for such documents. Second, a small fraction of documents accounts for the majority of retrieval requests. This
% allows us to cache the intermediate states of these frequently
% accessed documents to reduce the computational burden.

%\wenhao{we should evaluate CacheBlend and RAGCache, and infer which document the user feeds into the LLM}
%\textcolor{red}{@Zixuan}
\ignore{
In the current Retrieval-Augmented Generation (RAG) scenario, LLMs generate more specific and accurate responses by knowledge from existing documents or user-uploaded content. In such a scenario, the model will repeatedly use previously accessed documents on one hand, while on the other hand, a small subset of documents will be frequently used in certain specific contexts. Therefore, the KV cache reuse techniques, such as CacheBlend~\cite{yao2024cacheblend} and RAGCache~\cite{jin2024ragcache}, and semantic cache reuse techniques, such as Ollama~\cite{ollama-website} can significantly reduce the response time of the LLM system and increase its throughput. This section presents preliminary findings concerning the timing leakage in the RAG scenario.


\para{Inferring the queried document through KV cache reuse}
We conducted our evaluation on the CacheBlend inference framework~\cite{cacheblend-github}, which is built upon vLLM and supports KV cache reuse. Using the Multi-news dataset~\cite{multinews-github,Fabbri2019MultiNewsAL}, we selected documents with different content at various lengths and obtained ROC curves of response times when users queried a specific document, both with and without the document being cached. We selected 500 documents of different lengths and contents from the dataset through simple data processing. When testing the caching effect of documents of different lengths, we first uploaded one of these documents to the LLM. Then, we repeatedly used this document to query the LLM to obtain a dataset of response times for document cache hits. Additionally, we used the remaining documents, which differ from the target document, to query and obtain a dataset of response times for document cache misses. During the AUC calculation, we labeled the response times for document matches as 1 and those for document misses as 0, and plotted the ROC curves for both. The results, as shown in \autoref{fig:ragroc}, indicate that since document lengths in RAG scenarios are typically in the range of a few hundred words, it becomes apparent whether a document is cached. This could potentially allow for the identification of private documents used by other users.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/ragroc.png}
    \caption{Leakage profile of sharing documents in the RAG scenario, under different document sizes.}
    \label{fig:ragroc}
\end{figure}

% For example, we can first prepare 100 documents of same and different sizes, and plot the timing of querying the documents (such as: please summary the document) when the document hit or miss the cache. Then it will be obvious we can recover the private document.

\para{Inferring the visited website through semantic cache reuse}
Side-channel information leakage can occur when users on the same host access browsers and use the same LLM plugin. We examined Lumos, an LLM plugin designed to summarize web content and respond to queries. We found that the caching effect occurs when different users access the same web pages and send the same queries, resulting in timing side channels.
%This phenomenon indicates that we can exploit this feature to implement side-channel attacks.

Furthermore, we deployed an LLM locally that responds within web pages using Ollama~\cite{ollama-website}, with RedisCache and RedisSementicCache as the back-end cache. We queried the same prompts with different users in different browsers (e.g., Chrome and Edge) and found that there are significant time differences when the cache is hit, and the response time decreases from several seconds to milliseconds. This further proves the possibility of side-channel attacks.

\wenhao{We need to use RAG to demonstrate end-to-end attack on OpenAI's APIs, using image captioning or document asking}

\wenhao{maybe our case is not a typical RAG, and may change the title}
}

%\path{https://github.com/andrewnguonly/Lumos}
% 这个repo可以基于本地llm，通过chrome插件对网页内容进行总结
% 支持vector store，近期访问过的网页会被缓存
% 

%\textcolor{red}{@Zixuan please put the result here}


%\url{https://www.yuque.com/u19383/otg3d4/klwwx1ukmx2u5m4g}

%description: \path{https://medium.com/@andrewnguonly/local-llm-in-the-browser-powered-by-ollama-236817f335da}


% THIS DATA might be wrong, the setting is not right.

% one: TPR: 0.8670886075949367 FPR: 0.04219409282700422

% two tpr: 0.8510405257393209 fpr: 0.04819277108433735

% more than two TPR: 0.8837675350701403 FPR: 0.036072144288577156

%

%

% what's number here: more than 2?
% 3 or more than 3.

% Greedy way: no limit
% 0.8037865748709122 fpr: 0.03442340791738382

% Greedy way with limit for orthogonal sentences of length 2.
% tpr: 0.9273182957393483 fpr: 0.06015037593984962
% tpr: tpr: 0.8919540229885058 fpr: 0.06666666666666667

% Greedy way with limit for orthogonal sentences of length 3.
% tpr: 0.8408071748878924 fpr: 0.04484304932735426

% result:
% Greedy search with some limit, not too many will have great 
\ignore{
\begin{algorithm}[hbt!]
\caption{Semantic Searching Algorithm}\label{alg:semantic}
    \SetKwProg{Fn}{Function}{}{}

    \KwData{

    }

    \KwResult{
    }

    \SetKwFunction{TestSize}{TestSize}
    \SetKwFunction{GetSize}{GetSize}
    
    \Fn{\TestSize{Start, End, A, C, MT}}{
    }

    \Fn{\GetSize{}}{

    }


\end{algorithm}
}

%accuracy under different model temperature and similarity threshold

%In the experiments conducted in the real environment of GPTCache, the results demonstrate that we can successfully acquire the victim's prompt through an approach that involves evicting and attacking simultaneously, while also preventing the influence of the attacker's own input on the experimental outcomes, thereby enhancing the efficiency of the attacker's input prompts. Therefore, in practical applications, sensitive information input by users into LLMs may be captured by other malicious attackers, leading to the leakage of private data.


% goals: (1) use a public dataset to explain what can be leaked (2) understand the relationship between temprature and cache reuse
%(3) how to avoid the noise of caching the attacker's prompt




%A table showing at which step does the leakage locate, the targeted open-source project, what can be inferred

%\link{Mainly focusing on the serving part of this paper list.
%https://github.com/AmberLJC/LLMSys-PaperList}



==> tex/non-attacks.tex <==
\appendix

\section{Not-a-good Targets}

\subsection{Orion}
Orion~\cite{strati2024orion}

\link{I think Orion might not be our target, this paper seems mainly focusing on CUDA/CUDA-Kernel/GPU utilization and scheduling, guess it might a bit out of our scope.}

\subsection{AttentionStore}
See comment here
% https://arxiv.org/pdf/2403.19708
% 我在scholar中对sglang的引用中找到了这篇文章，看起来也是对多个request的共有部分进行加速的工作，发在今年的ATC会议上
\link{It's not a LLM work, in fact it is a storage work. Use different level of disk/cache/scheduling/pre-loading ways to store KV-Cache block into}

\para{Evaluations}

\subsection{Preemption}
SHEPHERD~\cite{zhang2023shepherd} provides guaranteed goodput under workload unpredictability by carefully leveraging preemptions and model-specific batching properties. similar work~\cite{han2022microsecond}\wenhao{they seem not a good target}
% https://www.usenix.org/system/files/nsdi23-zhang-hong.pdf

LLM preemptions: SpotServe (ASPLOS 2024)~\cite{miao2023spotserve} is also not a good target.

FastServe~\cite{wu2023fast} uses preemptive scheduling to minimize JCT with a novel skip-join Multi-Level Feedback Queue scheduler. Based on the new semi information-agnostic setting of LLM inference, the scheduler leverages the input length information to assign an appropriate initial queue for each arrival job to join. The higher priority queues than the joined queue are skipped to reduce demotions. We design an efficient GPU memory management mechanism that proactively offloads and uploads intermediate states between GPU memory and host memory for LLM inference.\wenhao{only leaks the priority, which does not contain sensitive information}

\subsubsection{Sharing intermediate blocks}
- beam search

\subsubsection{Copy on write}
When the attacker want to steal a victim's prompt (cached in the blocks), he can brute force short prompts and check response time => to observe if new physical KV blocks are created (assuming creating new KV blocks affects latency)
Assuming the attacker and the victim shares one half-filled block, when the attacker observes a sudden latency increase, he may know copy-on-write happens and therefore his next token is different from the victim's

\subsubsection{Prompt template sharing}

and modular prefix caching~\cite{gim2023prompt}



\para{Evaluations}

\subsubsection{Cascade Inference}
Cascade Inference: Memory Bandwidth Efficient Shared Prefix Batch Decoding: \url{https://flashinfer.ai/2024/02/02/cascade-inference.html}

In this blog post, we introduce Cascade Inference, which simply decouples attention of shared prefix and unique suffixes, and enables storing shared KV-Cache in GPU shared memory (SMEM for short) for fast access in multiple requests. We show that Cascade Inference can greatly accelerate shared-prefix batch decoding operator, with up to 31x speedup compared to the baseline vLLM PageAttention implementation and 26x speedup compared to FlashInfer batch decoding operator without cascading on a H100 SXM 80GB. The kernels have been supported in FlashInfer as PyTorch and C++ APIs.

\section{Summary}

\ignore{
\begin{table*}
    \centering
    \caption{Summary of KV cache reuse mechanisms.}
    \label{tab:my_label}
    {\small
    \begin{tabular}{C{3cm}C{2.8cm}C{2.6cm}C{2.8cm}C{2.8cm}}
    \hline 
             & Unit of shared tokens & Timing difference? & Automatic prefix sharing? & Cache-aware scheduling? \\ \hline
        SGlang~\cite{zheng2023efficiently,sglang-github} & 1 & yes & yes & yes\\ \hline
        vLLM~\cite{kwon2023efficient,vllm-github} & 8, 16 (default), 32 & yes & yes  &\\ \hline
        ChunkAttention~\cite{ye2024chunkattention,chunkattention-github} & $<128$ (default: 64) & yes & yes &\\ \hline
        vAttention~\cite{prabhu2024vattention,vattention-github} & 32, 64, 128, etc. (depending on GPU page size) & yes &  &\\ \hline
        %AttentionStore~\cite{gao2024attentionstore} &  &  &  &\\ \hline
    \end{tabular}
    }
\end{table*}
}
